Semi-decentralized Training of Spatio-Temporal Graph Neural Networks for Traffic Prediction

In smart mobility, large networks of geographically distributed sensors produce vast amounts of high-frequency spatio-temporal data that must be processed in real time to avoid major disruptions. Traditional centralized approaches are increasingly unsuitable to this task, as they struggle to scale with expanding sensor networks, and reliability issues in central components can easily affect the whole deployment. To address these challenges, we explore and adapt semi-decentralized training techniques for Spatio-Temporal Graph Neural Networks (ST-GNNs) in smart mobility domain. We implement a simulation framework where sensors are grouped by proximity into multiple cloudlets, each handling a subgraph of the traffic graph, fetching node features from other cloudlets to train its own local ST-GNN model, and exchanging model updates with other cloudlets to ensure consistency, enhancing scalability and removing reliance on a centralized aggregator. We perform extensive comparative evaluation of four different ST-GNN training setups -- centralized, traditional FL, server-free FL, and Gossip Learning -- on large-scale traffic datasets, the METR-LA and PeMS-BAY datasets, for short-, mid-, and long-term vehicle speed predictions. Experimental results show that semi-decentralized setups are comparable to centralized approaches in performance metrics, while offering advantages in terms of scalability and fault tolerance. In addition, we highlight often overlooked issues in existing literature for distributed ST-GNNs, such as the variation in model performance across different geographical areas due to region-specific traffic patterns, and the significant communication overhead and computational costs that arise from the large receptive field of GNNs, leading to substantial data transfers and increased computation of partial embeddings.

==> section_v1/0_abstract.tex <==
\begin{abstract}
The rapid growth of connected vehicles and smart infrastructure in the smart mobility domain generates massive amounts of traffic data for training deep learning models, making traditional centralized approach of data collection, storage and processing no longer suitable for this task. Centralized solutions face issues such as scalability, single points of failure, etc. While Federated Learning has emerged as a potential solution to this problem, it requires a central trusted aggregator to combine the contributions of different devices, and this cannot fully eliminate the aforementioned issues. To address these challenges, we explore and adapt semi-decentralized online training techniques for Spatio-Temporal Graph Neural Networks (ST-GNNs) to be used in the smart mobility domain. To achieve this, we implement a simulation framework that distributes nodes across multiple cloudlets, with each cloudlet training its own local ST-GNN model. This approach enhances scalability and eliminates the need for a centralized aggregator, resolving the issue of a single point of failure. We compare four different setups - centralized training, FL with an aggregator, server-free FL, and Gossip Learning - using large-scale traffic datasets from California and Los Angeles County, the METR-LA and PeMS-BAY datasets, for short-, mid-, and long-term vehicle speed predictions. Experimental results show that while centralized and FL with central aggregator setups achieve the highest predictive accuracy, server-free FL and Gossip Learning provide competitive results. In addition, despite taking longer to converge, Gossip learning offers the lowest communication overhead, making it a viable solution in smart mobility environments, providing a trade-off between scalability and convergence speed.


% Due to fast rise of increase in data availability for training deep learning models in smart mobility use-case, the traditional centralized approach of data collection, storage and processing is no longer suitable for this task. Additionally, centralized solutions face issues such as scalability, single points of failure, etc. To handle these issues, approach such as Federated Learning are being used. However, Federated Learning requires a central trusted aggregator to combine the contributions of different devices, and thus cannot fully eliminate the aforementioned issues. To address these limitations, we explore and adapt semi-decentralized online training techniques for Spatio-Temporal Graph Neural Networks (ST-GNNs) in smart mobility domain. Our framework distributes nodes across multiple cloudlets, each with its own local ST-GNN model, enabling better scalability and removing the need for a centralized aggregator, thus removing the issue of single point of failure. To the best of our knowledge, no previous work has attempted to implement semi-decentralized online training for GNNs that account for both spatial and temporal dependencies. We compare 4 different setups, including centralized, Federated Learning with centralized aggregator, server-free Federated Learning, and gossip learning, using the METR-LA and PeMS-BAY datasets for short, mid, and long-term vehicle speed predictions. Experimental results shows that (TBD).
\end{abstract}

==> section_v1/1_introduction.tex <==
\section{Introduction}
Smart mobility has emerged as a crucial research focus within urban planning \cite{cite_1}. Since its introduction, the concept has been increasingly applied to transportation systems, influencing both urban development and transport planning due to its innovative nature. One of key component of smart mobility is traffic prediction \cite{cite_2}, such as predicting the speed of vehicles, predicting the number of passengers using public transport, etc. As the significance of these services increases, there is a growing need for accurate and efficient forecasting of traffic patterns. Such forecasting enables effective management of transportation resources and allows for dynamic traffic control, minimizing congestion and reducing travel times. It also supports the optimization of routes, urban infrastructure, traffic flow, and public transportation planning.

In recent times, traffic forecasting has been receiving increasing attention \cite{cite_3, cite_4, cite_5, cite_6}. Like other prediction tasks, traffic forecasting methods can generally be divided into two primary categories. The first involves model-based approaches, where statistical models are used to represent traffic patterns, such as linear models. Although these model-based approaches are simple, they concentrate solely on temporal dependencies and overlook spatial dependencies, which are essential for achieving more accurate predictions. The second category includes Deep Learning (DL)-based approaches, where data-driven techniques have demonstrated an ability to efficiently leverage spatio-temporal correlations for enhanced prediction accuracy. In particular, Recurrent Neural Networks (RNN), such as Long Short-Term Memory (LSTM) \cite{cite_7} or Diffusion Convolutional Recurrent Neural Networks (DCRNN) \cite{cite_8} are crucial for traffic prediction due to their ability to handle time dependencies.

In order to further improve accuracy of predictions for traffic prediction, there has been increasing interest in applying Graph Neural Networks (GNNs), where nodes represent entities or individual data points in the graph, and edges represent the relationship or interactions between pairs of nodes. In the case of traffic prediction, each node typically represents a spatial location, such as a point on a map, and edges signify the spatial connections or dependencies between these locations. This representation allows GNN to capture spatial changes by considering the interconnectedness of nodes within the network. Several studies have highlighted the benefits of GNNs in leveraging local area information compared to RNNs \cite{cite_9, cite_10, cite_11}. To effectively model these dependencies, Spatio-Temporal Graph Neural Networks (ST-GNNs) have been developed, combining spatial capabilities of GNNs with temporal processing, allowing them to effectively model the complex interactions over time and space. Numerous ST-GNNs have been developed, such as Graph Recurrent Network (GRN) \cite{cite_12}, Spatio-Temporal Graph Convolutional Network (ST-GCN) \cite{cite_13}, Graph Attention LSTM Network \cite{cite_14}, Dynamic Spatio-Temporal Graph Neural Network \cite{cite_15}, and many more \cite{cite_16}. Each technique addresses specific challenges or offers unique advantages over others. In this work, ST-GCN will be used due to its superior ability to handle traffic prediction tasks compared to other techniques.

With the rise of connected vehicles and smart mobility infrastructure, modern cities are generating massive amounts of data that can be leveraged for intelligent traffic management. However, most solutions were developed in centralized or FL with centralized aggregator environment. Traditional centralized approaches to data collection and processing struggle to keep pace with the ever-increasing volume of data generated in real time. Centralized systems face scalability issues, privacy concerns, and single points of failure, which can lead to inefficiencies and even breakdowns in smart transportation networks. Additionally, the problem with FL is that it requires a central reliable aggregator to combine the contributions of different devices and therefore cannot completely eliminate scalability and reliability issues.

Based on the discussion above, in this paper, we explore and adapt online training techniques for Spatio-Temporal Graph Neural Networks (ST-GNNs) in smart mobility domain in a semi-decentralized way at the network edge, ensuring scalability, reliability and quick adaptation to local changes. This approach utilizes multiple cloudlet devices,  each responsible for managing a subgraph of the overall traffic graph. A cloudlet is a device with moderate computing power, positioned at a fixed location, capable of communicating with sensor nodes within its range as well as with other cloudlets. The contributions of this paper can be summarized as follows:

\begin{itemize}
\item We implement a simulation framework for distributed ST-GNN training across cloudlets, where each cloudlet independently trains a local model using data from nearby nodes. This setup avoids the need for a central aggregator, thereby improving system scalability and resilience to single points of failure.
\item We explore four training approaches to ST-GNN training for traffic prediction: centralized, FL with a central aggregator, server-free FL, and Gossip Learning. By comparing these approaches, we provide insights into their relative strengths and weaknesses, particularly in terms of accuracy, convergence speed, and communication costs.
\item We evaluate the performance of each approach on two large-scale real-world datasets, METR-LA and PeMS-BAY, for short-, mid-, and long-term traffic predictions. Our analysis includes a detailed examination of metric analysis, metric analysis of each individual cloudlet, convergence analysis, as well as model and node feature transfer analysis.
\end{itemize}

Experiments demonstrate that the server-free FL and Gossip Learning approaches achieved competitive accuracy relative to centralized and FL with central aggregator methods. For the METR-LA dataset, in short-term predictions, server-free FL and Gossip Learning achieved WMAPE scores of 8.89\% and 9.74\%, respectively, compared to 7.91\% for centralized setup and 8.01\% for FL with a central aggregator. For mid-term predictions, server-free FL and Gossip Learning achieved WMAPE scores of 12.51\% and 12.58\%, respectively, compared to 11.37\% for centralized setup and 11.67\% for FL with central aggregator. For long-term predictions, server-free FL and Gossip Learning achieved WMAPE scores of 16.76\% and 18.00\%, respectively, compared to 15.93\% for centralized setup and 16.08\% for FL with a central aggregator. %Now do PeMS-BAY

Additionally, despite talking the longest to converge compared to other semi-decentralized approaches, Gossip Learning offers the lowest model transfer cost, making it a viable solution in smart mobility environments, providing a trade-off between scalability and convergence speed.

% https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=10137765
% The rest of this paper is organized as follows. In Section II...

% --------------------------------------------------------------------------

% https://arxiv.org/pdf/2303.00524
% 1st paragraph:
% Talk about Smart mobility (is an essential item in modern city planning... A key component of smart mobility is traffic forecasting)
% then talk about traffic forecasting (taxi prediction, speed vehicles, number of passangers for public transports, etc.) -->say what are the benefits of accurate prediction

% 2nd paragraph:
% Traffic forecasting has been receiving increasing amounts of attention in  the recent literature (cite here). Just like other prediction problems, traffic prediction can be broadly categorized into two main categories: model based approach and deep learning based methods --> RNN such as LSTM is important for traffic prediction as they address time dependency (cite works here)

% 3rd paragraph:
% Talk about GNNs
% Talk about current problems (only centralized solutions, with some FL with centralized aggregator) --> say that online training hasn't been done in semi-decentralized environment

% 4th paragraph
% Based on the above discussion, in this paper, we (do stuff)
% The contributions of this paper can be summarized as follows: (list with dots)

% 5th paragraph
% Talk about solutions: "Experiments on real-world vehicle speed data show..."

==> section_v1/2_related-work.tex <==
\section{Related Work}
Training and testing GNN models on large graphs demand substantial memory and processing resources due to the interdependence of graph nodes. As a result, nodes cannot be easily split into smaller subgraphs. Even a sampled computational graph with its associated features might exceed the memory capacity of a single device \cite{cite_17}. This creates a scalability issues, privacy concerns, and single points of failure for centralized GNN operations \cite{cite_18}, especially when dealing with large-scale graphs or sensitive data collected from distributed sensors in real-time traffic prediction.

\subsection{Centralized ST-GNN training}\label{AA}
However, the majority of existing approaches for training ST-GNNs are based on centralized architectures \cite{cite_12, cite_13, cite_14, cite_15}. In such settings, the entire graph data is collected and processed at a central server, where models are trained and updated with full access to all nodes and their dependencies.

While this approach allows for the direct management of both spatial and temporal correlations, ensuring that the full context of the data can be leveraged to improve the models accuracy and performance, it comes with significant limitations as described above. First, the need to transfer all data to a central location presents considerable privacy and security risks, especially if data may include personal information or real-time tracking. Second, the scalability of centralized solutions is hindered by memory and computational constraints, as processing large graphs can overwhelm even high-capacity servers. And lastly, the reliance on a central server introduces a single point of failure, making the entire system vulnerable to downtimes.

\subsection{Federated Learning ST-GNN training}\label{AA}
To address these issues, Federated Learning (FL) \cite{cite_19} has emerged as an alternative, distributing the model training across multiple clients while using a central aggregator to combine the locally updated models. Several works have applied FL to train ST-GNN models for traffic prediction \cite{cite_20, cite_21, cite_22, cite_23}. This approach offers an improvement in data privacy, as raw data is kept locally and only model updates are shared with the aggregator. The central aggregator then combines these updates from various clients to form a global model, which is redistributed to the clients for the next round of training. This iterative process continues until the model converges.

One of the primary advantages of FL is its enhancement of data privacy. By keeping raw data on local devices or edge nodes, FL mitigates the risk of data breaches and privacy violations associated with transmitting sensitive information, such as location, personal habits, or traffic data, to a central server. FL also reduces communication overhead. Rather than sending large volumes of raw data over the network, which can cause congestion or delays, clients only transmit compressed model updates to the aggregator. This is especially beneficial in traffic prediction data where sensor nodes produce large amounts of data that are impractical to centralize.

While this approach improves on centralized training, it still relies on a central aggregator and thus shares some of the issues of a traditional centralized training. Furthermore, the central aggregator could potentially exploit its access to the received gradients to infer sensitive data. It might also intentionally manipulate the aggregation process, introducing biases that could affect the training procedure. Another challenge is scalability, as the aggregator needs to expand its network capacity and memory to accommodate all participants. Furthermore, it serves as a single point of failure, meaning that if the aggregator goes offline or is compromised, the entire training process can completely stop. Thus, FL cannot fully eliminate the issues of scalability, privacy, and single points of failure as described above.

\subsection{Decentralized and semi-decentralized ST-GNN training}
To the best of our knowledge, there has been no prior research specifically focused on decentralized or even semi-decentralized training of ST-GNNs for traffic prediction.

One relevant work by L. Giaretta et. al. \cite{cite_24} addresses decentralized online training. In their work, they address new challenges that arise in fully-decentralized scenario, and provide solutions to them. However, their solution is not tailored to ST-GNNs, but rather to Graph Convolutional Network (GCN), limiting its applicability to traffic prediction tasks that require both spatial and temporal correlations.

While there is no prior research work for decentralized online training for ST-GNNs, M. Nazzal et. al. \cite{cite_25} developed Heterogeneous Graph Neural Network with LSTM (HetGNN-LSTM) for taxi-demand prediction and tested it in a semi-decentralized environment, where nodes were partitioned into cloudlets, without any central aggregator, thereby enhancing scalability and reliability. However, their solution only enables semi-decentralized inference by deploying a pre-existing model, with no support for online semi-decentralized training. Building on the foundations of this semi-decentralized inference work, our research will investigate and extend these ideas to enable semi-decentralized online training of ST-GNNs. Specifically, this paper will explore and adapt techniques such as server-free FL and gossip learning to train ST-GNN models in a semi-decentralized manner. These approaches will be evaluated and compared against centralized and FL with a central aggregator to determine their effectiveness for traffic prediction tasks.

% Talk about Giaretta work about decentralized online training -> say that it's not for spatio temporal GNN

% Then talk about semi-dec inference work, but say that it's inference and that this paper will work on semi-dec online training based on their work???
    % Hence this work will explore and adapt semi-dec online training tecniques for SP-GNNs such as server-free FL or gossip learning and compare them to centralized and FL with central aggregator

==> section_v1/3_preliminary.tex <==
% https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=10137765
% https://www.sciencedirect.com/science/article/abs/pii/S156849462300193X
\section{Preliminary}
\subsection{Traffic prediction}
Smart mobility encompasses a wide range of tasks aimed at improving transportation systems, such as route optimization, congestion management, and traffic prediction. Among these, traffic prediction is one of the most common and critical time-series forecasting tasks, as it estimates the most probable traffic metrics, such as speed, volume, and density, which are typically used to monitor current traffic conditions and predict future trends. While our focus in this work is on traffic prediction, many methods and models developed for other smart mobility tasks can be generalized to this domain due to their shared reliance on spatio-temporal data.

Based on the prediction horizon, traffic forecasting is generally classified into three scales: short-term (15 min), medium-term (30 min), and long-term (60 min). In this context, the traffic system is represented as a spatial graph at the \textit{t}-th time step, denoted by $\mathcal{G}_t$ = ($\mathcal{V}_t$, $\mathcal{E}$, W), where $v_i, v_j\in \mathcal{V}_t$ is a finite set of nodes corresponding to observations from \textit{n} IoT-devices in the traffic network, $(v_i, v_j)\in \mathcal{E}$ is a set of edges connecting the IoT-devices, and $W\in \mathbb{R}^{n x n}$ is a weighted adjacency matrix that encodes the spatial relationships between these IoT-devices. The spatial component of this graph is defined by the actual physical location of the IoT-devices, represented by the nodes $\mathcal{V}_t$, and the set of edges $\mathcal{E}$ connecting them. Meanwhile, the temporal component arises from the evolving traffic features recorded by the IoT-devices over time, which vary at each time step and influence the dynamics of the graph.

\begin{comment}
\subsection{Spatio-Temporal Graph Convolutional Network}
The model used in this paper is the Spatio-Temporal Graph Convolutional Network (ST-GCN) due to their superior ability to handle traffic prediction tasks in the IoT context compared to other techniques that use RNN-based models since RNN-based models still suffer from time-consuming iterations, complex gate mechanisms, and slow response to dynamic changes. Instead of RNN, they employed the entire convolutional structures on time axis to capture temporal dynamic behavior. This speciﬁc design allows parallel and controllable training procedures through multi-layer convolutional structures formed as hierarchical representations \cite{cite_13}.
\end{comment}

\subsection{Spatio-Temporal Graph Neural Networks}
Spatio-Temporal Graph Neural Networks (ST-GNNs) are DL models designed to capture both spatial and temporal dependencies in structured data. The ability to capture both spatial and temporal dependencies enables the model to simultaneously account for spatial correlations between nodes and temporal correlations over time, making it particularly suited for spatio-temporal forecasting tasks like traffic prediction.

Multiple ST-GNNs have been developed \cite{cite_16}, and each technique addresses specific challenges or offers unique advantages over others. The model used in this paper is the Spatio-Temporal Graph Convolutional Network (ST-GCN) due to their superior ability to handle traffic prediction tasks in the IoT context compared to other techniques. ST-GCN model achieves the best performance with statistical signiﬁcance in all evaluation metrics (MAE, MAPE, and RMSE) \cite{cite_13}.

\subsection{Server-free Federated Learning}
Server-free FL \cite{cite_26} is a decentralized variation of the traditional FL approach. Unlike standard FL, where a central server or aggregator is responsible for coordinating the model updates, server-free FL operates without a central entity. Instead, participating devices communicate directly with one another to exchange model parameters and perform local updates.

After initializing their models, devices exchange model parameters with their neighbors, aggregate these received models with their own local model, and proceed to train on subset of data. This iterative process allows for continuous refinement of models across the network, as the updated models are exchanged again between neighbouring devices.

One of the key advantages of this approach is its resilience to the single points of failure, as there's no central server coordinating the process, unlike centralized or traditional FL approaches, enhancing both scalability and resilience by enabling decentralized, peer-to-peer collaboration among devices.

However, in order to maintain consistency, this approach relies on the assumption that devices can communicate reliably and operate in a mutually trusted environment, so devices can reliably share models without the need for a central authority.
\begin{comment}
    In order to train ST-GNNs in a distributed manner, we employ server-free FL \cite{cite_26}. Server-free FL works similarly to FL, however no central server is present to coordinate model updates. Instead, cloudlets communicate directly with one another, exchanging and aggregating models locally in a decentralized manner. Each cloudlet acts as an individual FL client, responsible for both training and communication.

    In this setting, after initializing their models, cloudlets exchange model parameters with their neighbors, aggregate these received models with their own local model, and proceed to train on their local data. This iterative process allows for continuous refinement of models across the network, as the updated models are exchanged again between adjacent cloudlets. Unlike traditional FL that relies on a central aggregator, this server-free FL approach eliminates the need for a single point of control, enhancing both scalability and resilience by enabling decentralized, peer-to-peer collaboration among cloudlets.

    To maintain consistency, it is assumed that neighboring cloudlets operate in a mutually trusted environment, where they can reliably share models without the need for a central authority. This decentralized structure allows for more flexible and dynamic model updates, while still benefiting from the collective knowledge of the entire traffic network. Each cloudlet's contribution is based on the local traffic patterns it observes, allowing the system to quickly adapt to regional changes while still improving the overall model for traffic prediction.
\end{comment}

% Figure 1
\begin{figure*}[ht!]
  \centering
  \includegraphics[width=1\linewidth]{figures/semi-dec-st-gcn-arch.drawio.png}
  \caption{Semi-decentralized ST-GCN architecture}
  \label{fig:1}
\end{figure*}

\subsection{Gossip Learning}
Gossip learning \cite{cite_27} is a decentralized, peer-to-peer protocol for training machine learning models in distributed settings without the need for a central coordinator. It is designed to be highly scalable and robust, allowing model updates to be propagated efficiently across a network of devices or nodes.

Each device stores two models in its memory (as a FIFO buffer), typically representing the most recent models received from neighboring devices. At each iteration of the gossip protocol, a device averages the weights of these two models to create an aggregated model. The device then performs one local training step using its own data, refining the aggregated model based on its local observations. Once the model is updated, the device forwards it to a randomly selected neighboring device in the network. This process is repeated across the network, ensuring that models continuously evolve and improve as they traverse different nodes, collecting knowledge from the data they encounter at each location.

Just like server-free FL, a key advantage of gossip learning is its resilience to failures. Additionally, it allows very fast and efficient information propagation and thus results in quick convergence.
\begin{comment}
    In addition to server-free FL, we employ gossip learning \cite{cite_27} as a decentralized, peer-to-peer protocol to train ST-GNNs in a distributed manner. Gossip learning is very robust and scalable, and it efficiently propagates model updates efficiently without relying on a central coordinator.

    Each cloudlet stores two models in its memory (as a FIFO buffer), representing the most recent models received from neighboring cloudlets. At each iteration of the gossip protocol, the cloudlet averages the weights of these two models to form an aggregated model, performs a local training step using its local traffic data, and forwards the newly updated model to a randomly selected neighboring cloudlet. This ensures that models evolve continuously as they traverse the network, picking up information not only from their current node but also from the prior knowledge obtained from other cloudlets they visited.

    Just like server-free FL, a key advantage of gossip learning is its resilience to failures. Additionally, its low communication complexity makes it suitable for resource-constrained environments like smart mobility systems, where cloudlets have limited bandwidth or computational power.
\end{comment}


==> section_v1/4_methodology.tex <==
\section{Methodology}
% Start the section with the scenario

% Talk that online training is important - but if we don't do it, then don't claim that our approach is online training (it's distributed training)

% Focus is the distributed online training
%   -> Before methodology (Preliminary section) -> maybe a better name for section
%   -> There are a lot of task in Smart mobility, but we focus on "traffic prediction task" and other taks can generalize to them
%   -> talk about why it's spatio temporal (explain what is spatio temporal, what are the components in the traffic prediction)
%   -> Talk about "ST-GNNs", but we implement 1 ST-GCN because of tests it's better
%   -> What are key metrics for this tasks

% In methodology -> maybe a better name for section
%   -> start talking about infrastrucuture - the data is coming from sensors, and BS collect these sensors using LoRa
In this study, we explore four different approaches for distributed training of ST-GNNs for traffic prediction: centralized training, FL with a central aggregator, server-free FL, and gossip learning. The experiments are performed using real-world traffic datasets from California and Los Angeles County (METR-LA and PeMS-BAY) for short, mid, and long-term vehicle speed prediction.

\subsection{Scenario and Infrastructure}
The traffic prediction scenario involves IoT-devices (i.e. sensors) deployed along highways to monitor real-time traffic conditions. Each IoT-device records traffic metrics such as vehicle speed, volume, and density at fixed time intervals. These IoT-devices are partitioned to a local base stations (i.e. cloudlets), based on their physical proximity and the communication range. The communication between IoT devices and cloudlets is achieved through the Low-Power Wide-Area Network protocol, such as LoRa, which enables efficient, long-range data transmission.

\paragraph{Cloudlet architecture and data collection}
Our method leverages local cloudlets, similar to the work of Nazzal et al \cite{cite_25}, where each cloudlet is a computing node with moderate processing power, responsible for collecting and processing data from its partitioned IoT-devices, and training it's local ST-GNN model. As shown in Fig.~\ref{fig:1}, cloudlets form a semi-decentralized architecture where:

\begin{itemize}
\item IoT-devices send traffic data to their partitioned cloudlet
\item Cloudlets train local ST-GNN models on the received data, capturing both the spatial and temporal patterns of the traffic
\item Cloudlets send node features of its partitioned IoT-devices to other cloudlets for local training purposes
\item Cloudlets communicate with other cloudlets to exchange model updates in decentralized scenarios such as server-free FL and gossip learning
\end{itemize}

\subsection{Approaches for ST-GNN training}
\paragraph{Centralized training}
In the centralized training approach, all IoT-device data is collected by a central server, which aggregates the data and trains a global ST-GNN model. This setup ensures the model has full access to the entire traffic network, enabling it to learn comprehensive spatial and temporal correlations. This approach will serve as a baseline for comparing more distributed approaches.

\paragraph{Federated Learning with central aggregator}
In the FL with central aggregator approach, each cloudlet trains its own local ST-GNN model based on its locally collected traffic data, with an additional traffic data from other cloudlets, depending on how many layers ST-GNN model has. The local model updates are sent to a central aggregator, which combines these updates to form a global model. This global model is then distributed back to the cloudlets for further rounds of training.

\paragraph{Server-Free Federated Learning}
Server-Free FL is a decentralized training approach that works similarly to FL with central aggregator. However, this approach eliminates the need for a central aggregator, enabling direct communication between neighbouring cloudlets. After local training, each cloudlet shares its updated model with its neighboring cloudlets. These neighboring cloudlets aggregate the received model updates with their own local model and proceed with further training. This process continues iteratively across the network.

\paragraph{Gossip Learning}
Gossip learning is another decentralized training approach where cloudlets exchange and aggregate models in a peer-to-peer fashion. Each cloudlet stores two models (received from other cloudlets) in a FIFO buffer. At each iteration, cloudlet averages the weights of the two models in the buffer, performs one step of local training of the aggregated model, and then forwards the updated model to a randomly-chosen cloudlet. This process ensures continuous model refinement as updates propagate across the network.

From a different perspective, each model behaves as if it's moving randomly across a fully connected communication graph. With every step, the model doesn't just update based on the data from the current cloudlet; it also incorporates knowledge gathered by the model that visited the device beforehand.
% Cloudlets collect traffic data from IoT-devices deployed across a highway. IoT-devices are partitioned into cloudlets based on distance to each cloudlet and communication range of each cloudlet. IoT-devices cannot be partitioned to multiple different cloudlets. These IoT-devices communicate with base stations using Low-Power Wide-Area network (i.e. LoRa) protocol, which allows efficient communication over long distances.

% As shown in Fig.~\ref{fig:1}, each cloudlet is responsible for collecting local traffic data and sending the data to other cloudlets. Cloudlets, which are computing devices with moderate processing power, train local ST-GNN models on the data they receive. The cloudlets communicate with each other to exchange model updates in decentralized scenarios, such as server-free FL and gossip learning.

==> section_v1/5_experiments.tex <==
\section{Experiments}
In this section, we present the results of our extensive experiments to evaluate different approaches for distributed training of ST-GNNs in the context of smart mobility using two real-world traffic datasets. Through these comparisons, we aim to demonstrate the effectiveness of semi-decentralized training techniques in addressing the scalability and reliability in traffic prediction, while maintaining high prediction accuracy.

\subsection{Dataset}
To evaluate the performance of our setups, we utilize two real-world public traffic datasets, PeMS-BAY and METR-LA, which are collected by Caltrans performance measurement system. Both datasets consist of traffic data aggregated in 5-minute intervals, with each sensor collecting 288 data points per day. The details of datasets are listed in Table~\ref{table:1}.

% TABLE I
\begin{table}[htbp]
    \centering
    \caption{Details of METR-LA and PeMS-BAY}
    \begin{tabular}{c c c c c}
        \hline
        Datasets & Nodes & Interval & TimeSteps & Attribute \\
        \hline
        METR-LA & 207 & 5 min & 34,272 & Traffic speed \\
        PeMS-BAY & 325 & 5 min & 52,116 & Traffic speed \\
        \hline
    \end{tabular}
    \label{table:1}
\end{table}

The spatial adjacency network is constructed from the actual road network based on distance using the formula from ChebNet \cite{cite_28}. Additionally, the data were preprocessed for efficient model training and evaluation. For example, if we want to utilize the historical data spanning one hour to predict the data the next hour, we pack the sequence data in group of 12 and convert it into an instance. The dataset was then split into training, validation, and test sets in a 7,5:1,5:1,5 ratio. Additionally, to mitigate the impact of varying data magnitudes, we applied Z-score normalization to standardize the original data values, reducing the impact of the large difference in value:

\begin{equation}
    Z_{score}(X) = \frac{X - mean(X)}{std(X)}
\end{equation}

\subsection{Evaluation Metrics}
In our experiments, we use three commonly adopted metrics for traffic forecasting to evaluate the performance of the different setups: mean absolute error (MAE), root mean square error (RMSE), and weighted mean absolute percentage error (WMAPE). The formulas are as follows:

\begin{itemize}
\item Mean Absolute Error (MAE): \\
\begin{equation}
    \text{MAE}(\bm{x}, \bm{\hat{x}}) = \frac{1}{n} \sum_{i} \mid x_i - \hat{x}_i \mid
\end{equation}

\item Root Mean Square Error (RMSE): \\
\begin{equation}
    \text{RMSE}(\bm{x}, \bm{\hat{x}}) = \sqrt{\frac{1}{n} \sum_{i} {(x_i - \hat{x}_i)}^2 }
\end{equation}

\item Weighted Mean Absolute Percentage Error (WMAPE): \\
\begin{equation}
    \text{WMAPE}(\bm{x}, \bm{\hat{x}}) = \frac{\sum_{i}{\mid x_i - \hat{x}_i \mid}}{\sum_{i}{\hat{x}_i}} * 100\%
\end{equation}

\end{itemize}

Where $\bm{x} = x_1,...,x_n$ denotes the ground truth values of vehicle speed, and $\bm{\hat{x}} = \hat{x}_1,...,\hat{x}_n$ represents their predicted values.

% Figure 2
\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{figures/locations_cloudlet.drawio.png}
  \caption{Sensor partitioning to cloudlets based on communication range. a) METR-LA. b) PeMS-BAY}
  \label{fig:2}
\end{figure}

\subsection{Experiment Settings}

% TABLE II
\begin{table*}[ht!]
\centering
\caption{Performance Comparison (MAE/RMSE/WMAPE [\%]) of four different setups}
\label{table:2}
\renewcommand{\arraystretch}{1.5} % Adjust row spacing for better readability
\begin{tabular}{l l ccc | ccc | ccc}
\hline\hline
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Setups} & \multicolumn{3}{c|}{15 min} & \multicolumn{3}{c|}{30 min} & \multicolumn{3}{c}{60 min} \\ 
\cline{3-11}
\multicolumn{2}{l}{} & MAE & RMSE & WMAPE (\%) & MAE & RMSE & WMAPE (\%) & MAE & RMSE & WMAPE (\%) \\ 
\hline\hline
\multirow{4}{*}{METR-LA} & Centralized             & 3.78 & 9.05      & 7.45 & 5.14 & 11.61       & 10.12 & 7.35 & 14.59      & 14.47 \\ \cline{3-11}
                                      & Traditional FL      & 3.97 & 9.01       & 7.82 & 5.40 & 11.41       & 10.63 & 7.82 & 14.48      & 15.40 \\ \cline{3-11}
                                      & Server-free FL          & 3.96 & 9.03       & 7.98 & 5.34 & 11.42      & 10.94 & 7.92 & 14.46      & 15.95 \\ \cline{3-11}
                                      & Gossip Learning         & 3.94 & 9.08      & 7.95 & 5.52 & 11.41      & 11.12 & 7.7 & 14.48      & 15.52 \\ 
\hline\hline
\multirow{4}{*}{PeMS-BAY} & Centralized             & 1.48 & 3.09      & 2.38 & 1.97 & 4.23      & 3.17 & 2.59 & 5.41      & 4.17 \\ \cline{3-11}
                                       & Traditional FL      & 1.50 & 3.12      & 2.42 & 2.03 & 4.29      & 3.27 & 2.67 & 5.51      & 4.29 \\ \cline{3-11}
                                       & Server-free FL          & 1.50 & 3.12      & 2.42 & 2.01 & 4.28      & 3.25 & 2.67 & 5.50      & 4.31 \\ \cline{3-11}
                                       & Gossip Learning         & 1.51 & 3.13      & 2.44 & 2.03 & 4.31      & 3.28 & 2.66 & 5.45      & 4.29 \\ 
\hline\hline
\end{tabular}
\end{table*}

All experiments were run multiple times with fixed 75 epochs, utilizing the High-Performance Computing (HPC) system Leonardo Booster, which features 4x NVIDIA A100 SXM6 64GB GPUs. The software environment used for the experiments included Python 3.10.14, PyTorch 2.3.1, and PyTorch Geometric 2.5.3.

For model architecture, we set the number of spatio-temporal blocks (ST-blocks) to 2, and used the GLU activation function. The learning rate was fixed at 0.0001, the dropout rate at 0.5, and the weight decay rate at 0.00001. A batch size of 32 was employed, MAE is used as the training loss, and Adam was chosen as the optimization algorithm. The temporal and spatial kernel size was set to 3 for all experiments, with Chebyshev convolution as convolutional layer. Learning rate scheduler was applied with the StepLR strategy, where the step size was set to 5, and the decay factor, gamma, was set to 0.7. All experiments use 60 minutes as the historical time window, a.k.a. 12 observed data points.

Additionally, sensors were distributed across 7 cloudlets based on proximity and communication range. Each cloudlet can communicate up to a maximum of 8 km. Fig.~\ref{fig:2} illustrates how sensors are partitioned into these cloudlets and their respective communication ranges for both the METR-LA and PeMS-BAY datasets. This partitioning reflects the semi-decentralized structure used for our distributed training approach.

\subsection{Experimental Results}

\paragraph{Setup metric analysis}
Table~\ref{table:2} shows the performance comparison of four different approaches for traffic speed prediction over three forecast horizons for two benchmark datasets, METR-LA and PeMS-BAY. For server-free FL and Gossip Learning, performance metrics were averaged across all cloudlets.

The results indicate a performance gap for WMAPE between centralized and semi-decentralized approaches, particularly as the forecast horizon increases, while MAE and RMSE stay relatively the same across all forecast horizons for all setups. For short-term predictions, this gap is relatively small. However, as the prediction horizon increases, the accuracy degradation becomes more pronounced.

This trend highlights the trade-off between accuracy and the enhanced scalability and resilience provided by semi-decentralized approaches. While centralized approach achieved the lowest error rates across most metrics, server-free FL and Gossip Learning are viable alternatives, particularly in scenarios where eliminating a central aggregator is essential for scalability and fault tolerance in distributed traffic prediction settings.

\paragraph{Cloudlet metric analysis}
% Figure 3
\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{figures/plot_val_metric_WMAPE_metr-la_cloudlet_subplot.png}
  \caption{WMAPE for individual cloudlets for METR-LA dataset}
  \label{fig:3}
\end{figure}

% Figure 4
\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{figures/plot_val_metric_WMAPE_pems-bay_cloudlet_subplot.png}
  \caption{WMAPE for individual cloudlets for PeMS-BAY dataset}
  \label{fig:4}
\end{figure}

% Figure 5
\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{figures/plot_val_metric_WMAPE_metr-la_pems-bay_cloudlet_subplot.png}
  \caption{WMAPE for individual cloudlets in centralized setup}
  \label{fig:5}
\end{figure}

Figures~\ref{fig:3} and~\ref{fig:4} presents the variability in WMAPE across cloudlets for Gossip Learning and Server-free FL for METR-LA and PeMS-BAY datasets, across prediction horizons of 15, 30, and 60 minutes, showing us a noticeable trend is the difference in performance between individual cloudlets in both approaches.

There's a significant spread in WMAPE values among cloudlets. For METR-LA dataset, cloudlet 5 performed the best, whereas cloudlets 1 and 7 performed the worst across all prediction horizons. For PeMS-BAY, cloudlets 6 and 7 performed the best, while cloudlets 1, 3 and 4 performed the worst across all prediction horizons. This is due to cloudlets location, and by extension, sensor partitioning. Figure~\ref{fig:5} shows WMAPE for each cloudlet in centralized setup. The model was trained just like in centralized setup. However, sensors were also partitioned to cloudlets in the same way it was done in other distributed setups, meaning that each cloudlet calculates WMAPE using the same model. From the figure, we can see that WMAPE for each cloudlet matches the ones from server-free FL and Gossip Learning.
% For example, in all experiments, cloudlet 5 achieved the best performance, while cloudlet 1 achieved the worst performance across all cloudlet. This is due to sensor partitioning. Figure~\ref{fig:5} shows WMAPE for each cloudlet in centralized setup. The model was trained just like in centralized setup, however sensors were also partitioned to cloudlets in the same way it was done in other distributed setups, so each cloudlet calculates WMAPE using the same model. From the figure, we can see that WMAPE for each cloudlet matches the ones from server-free FL and Gossip Learning.
% This is due to sensor partitioning and cloudlet location, as shown in Figure~\ref{fig:2}.
% Additionally, in some experiments, cloudlet 7 exhibits the same WMAPE as cloudlet 1, while in others it's much closer to cloudlet 2, 3, 4, and 6. These differences can be attributed to the experiments being initialized randomly, leading to slight variations in cloudlet performance across different runs.

\paragraph{Convergence analysis}

% Figure 6
\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{figures/plot_val_loss_metr-la_pems-bay_multi_subplot.png}
  \caption{Validation loss over epochs}
  \label{fig:6}
\end{figure}

Figure~\ref{fig:6} shows the validation loss curves for all four different approaches across three different forecast horizons for both METR-LA and PeMS-BAY datasets.

From the validation loss curves, we observe that the centralized approach consistently converges faster and achieves lower overall loss across all three forecast horizons. In contrast, FL with central aggregator and server-free FL exhibit same convergence rates, whereas Gossip Learning exhibit slowest convergence rate across all horizon predictions for both datasets. Gossip Learning, in particular, shows higher variability during validation, which reflects the challenges of decentralized learning. However, despite the slower convergence and higher initial volatility, all semi-decentralized approaches eventually reach reasonably low loss values, with only a marginal difference compared to their centralized counterpart. This suggests that while fully centralized methods may offer quicker convergence, semi-decentralized methods remain viable alternatives in traffic prediction environments, providing a trade-off between scalability and convergence speed.

\paragraph{Model and node feature transfer analysis}
% TABLE III
\begin{table}[htbp]
    \centering
    \caption{Average model and node feature transfer size per epoch per cloudlet}
    \label{table:3}
    \renewcommand{\arraystretch}{1.5} % Adjust row spacing for better readability
    \begin{tabular}{l l c | c}
    \hline\hline
    \multirow{1}{*}{Dataset} & \multirow{1}{*}{Setups} & \multicolumn{1}{c|}{Model [MB]} & \multicolumn{1}{c}{Node feature [MB]} \\ 
    % Header row
    %\multicolumn{2}{l}{} & Model [MB] & Node feature [MB] \\ 
    \hline\hline
    % METR-LA rows
    \multirow{4}{*}{METR-LA} 
        & Centralized              & - & 0.68 \\ \cline{3-4}
        & Traditional FL & 0.13 & 3.69 \\ \cline{3-4}
        & Server-free FL           & 0.23 & 3.69 \\ \cline{3-4}
        & Gossip Learning          & 0.13 & 3.69 \\ 
    \hline\hline
    % PeMS-BAY rows
    \multirow{4}{*}{PeMS-BAY} 
        & Centralized              & - & 1.61 \\ \cline{3-4}
        & Traditional FL & 0.13 & 9.44 \\ \cline{3-4}
        & Server-free FL           & 0.23 & 9.44 \\ \cline{3-4}
        & Gossip Learning          & 0.13 & 9.44 \\ 
    \hline\hline
    \end{tabular}
\end{table}

% The analysis of model and node feature transfer highlights the communication overhead between various training approaches. As shown in Table~\ref{table:3}, centralized training does not involve model transfer between nodes, since all computations occur in a single location. However, node feature transfers are necessary. Instead of sending node features to multiple cloudlets, they're being sent to one centralized system, amounting to 4.73 MB per epoch for the METR-LA dataset and 11.30 MB per epoch for the PeMS-BAY dataset.

The model and node feature transfer analysis highlights the differences in communication overhead between various training approaches. As seen in Table~\ref{table:3}, centralized training does not involve any model transfer between nodes, as all computations occur in a single location, while distributed systems such as FL with a central aggregator, server-free FL, and Gossip Learning require periodic model transfers during training.

FL with a central aggregator incurs a model transfer of 0.13 MB per epoch, as each cloudlet sends it's local model once to central aggregator per epoch. Gossip Learning also incurs a model transfer of 0.13 MB per epoch, as nodes share model updates only once per epoch to a random cloudlet in a network. Server-free FL shows a slightly lower transfer size of 0.23 MB per epoch. Theoretically, the model transfer size could be as large as $cln\_num * (cln\_num - 1) * Model [MB]$ if every cloudlet communicated with every other cloudlet in the network. However, due to the limited communication range of cloudlets, this theoretical upper bound is not reached. As we've seen in Fig.~\ref{fig:6}, it takes Gossip Learning the longest to converge. However, due to small model size, Gossip Learning is a viable option for traffic prediction environment using LPWAN communication protocols, such as LoRa.

Additionally, node feature transfers are necessary for each setup. In centralized setup, instead of node features being sent to each individual cloudlet, they're being sent to one centralized system, amounting to 4.73 MB per epoch for METR-LA dataset and 11.30 MB per epoch for PeMS-BAY dataset, or 0.68 MB per epoch per cloudlet for METR-LA dataset and 1.61 MB per epoch per cloudlet for PeMS-BAY dataset. For distributed setups, node feature transfer differs. On average, each cloudlet transfers 3.69 MB worth of node features per epoch for METR-LA dataset, or 25.84 MB in total per epoch. For PeMS-BAY dataset, each individual cloudlets transfers on average 9.44 MB worth of node features, or 66.10 MB in total per epoch. Each distributed setups transfer the same amount of node features since partitioning of the nodes to the cloudlets hasn't changed.

\begin{comment}
% Put them in Experiment (it's own subsection called "Evalation Metrics")
To evaluate the performance of each training approach, we use the following metrics:

\begin{itemize}
\item Mean Absolute Error (MAE) \\
\begin{equation*}
    \text{MAE}(\bm{x}, \bm{\hat{x}}) = \frac{1}{n} \sum_{i} \mid x_i - \hat{x}_i \mid
\end{equation*}

\item Root Mean Square Error (RMSE) \\
\begin{equation*}
    \text{RMSE}(\bm{x}, \bm{\hat{x}}) = \sqrt{\frac{1}{n} \sum_{i} {(x_i - \hat{x}_i)}^2 }
\end{equation*}

\item Weighted Mean Absolute Percentage Error WMAPE) \\
\begin{equation*}
    \text{WMAPE}(\bm{x}, \bm{\hat{x}}) = \frac{\sum_{i}{\mid x_i - \hat{x}_i \mid}}{\sum_{i}{\hat{x}_i}}
\end{equation*}

\item Training time: The time taken to train the model to convergence

\end{itemize}

Where $\bm{x} = x_1,...,x_n$ denotes the ground truth values of vehicle speed, and $\bm{\hat{x}} = \hat{x}_1,...,\hat{x}_n$ represents their predicted values.
\end{comment}

==> section_v1/6_future_work.tex <==
\section{Future Work}
\paragraph{Network communication}
One potential area for future work exploration is to explore methods to reduce communication overhead between cloudlets by focusing on model size optimization and connectivity adjustments. One approach involves leveraging model pruning techniques to create more compact versions of the ST-GNN models, which would decrease the model parameters and thus reduce the data transfer requirements for semi-decentralized methods. Additionally, instead of using distance-based edge connectivity, direct edge connectivity could be adopted to streamline the communication pathways, reducing the overall node feature transfer size per cloudlet.

By reducing both model and communication sizes, we aim to maintain or improve overall accuracy while minimizing the communication load. To evaluate the effectiveness of these techniques, we will compare model performance metrics, both with and without these optimizations, allowing us to gauge the trade-offs between communication efficiency and predictive accuracy.

\paragraph{Cloudlet personalization}
Another promising direction is implementing individual cloudlet personalization to address performance variability across cloudlets. Our results have highlighted a notable gap in error rates, especially in certain cloudlets with consistently higher WMAPE values. Personalizing cloudlets that have lower accuracy compared to the rest of the cloudlets, tailoring them to local traffic conditions or unique spatial-temporal patterns, could help reduce these disparities. Such a personalized approach may involve adjusting model parameters or incorporating local fine-tuning for cloudlets with higher error rates, potentially enhancing prediction accuracy across the network while maintaining decentralized resilience.

==> section_v1/7_conclusion.tex <==
\section{Conclusion}
In this paper, we have explored semi-decentralized approaches for traffic prediction in the smart mobility domain, comparing centralized, FL with a central aggregator, server-free FL, and Gossip Learning setups. By distributing ST-GNN training across multiple cloudlets, we aimed to address scalability and resilience challenges associated with traditional centralized approaches. Experimental results on the METR-LA and PeMS-BAY datasets demonstrate that server-free FL and Gossip Learning achieve competitive accuracy for all prediction horizons.

Our findings indicate that while centralized yielded the best accuracy, the semi-decentralized approaches, particularly server-free FL and Gossip Learning, offer viable alternatives with enhanced scalability and elimination of single points of failure. The trade-offs in prediction accuracy, highlight areas for further optimization, such as communication efficiency and model personalization, which we have proposed as directions for future work. Overall, this study contributes to the development of resilient and scalable traffic prediction solutions, supporting the evolving needs of smart mobility systems.

==> section_v2/0_abstract.tex <==
\begin{abstract}
%In the smart mobility domain, large networks of geographically distributed sensors produce vast amounts of high-frequency spatio-temporal data, which need to be processed in real time to prevent major disruptions. Traditional centralized approaches are increasingly unsuitable to this task, as it's difficult to scale them with the constantly-expanding sensor networks, and reliability issues in central components can easily affect the whole deployment. To address these challenges, we explore and adapt semi-decentralized training techniques for Spatio-Temporal Graph Neural Networks (ST-GNNs) in smart mobility domain. To achieve this, we implement a simulation framework that groups sensor nodes across multiple cloudlets based on their geographic proximity to a cloudlet. Each cloudlet handles a subgraph of the traffic graph, fetches node features from other cloudlets to train its own local ST-GNN model and exchanges model updates with other cloudlets to ensure consistency. This approach enhances scalability and eliminates the need for a centralized aggregator, resolving the issue of reliability. We perform extensive comparative evaluation of four different ST-GNN training setups---centralized, traditional FL, server-free FL, and Gossip Learning---using large-scale traffic datasets, the METR-LA and PeMS-BAY datasets, for short-, mid-, and long-term vehicle speed predictions. Experimental results show that semi-decentralized setups are comparable to centralized approaches in performance metrics, while offering advantages in terms of scalability and fault tolerance. In addition, we highlight often overlooked issues in existing literature for distributed ST-GNNs, such as the variation in model performance across different geographical areas due to region-specific traffic patterns, and the significant communication overhead and computational costs that arise from the large receptive field of GNNs, leading to substantial data transfers and increased computation of partial embeddings.

In smart mobility, large networks of geographically distributed sensors produce vast amounts of high-frequency spatio-temporal data that must be processed in real time to avoid major disruptions. Traditional centralized approaches are increasingly unsuitable to this task, as they struggle to scale with expanding sensor networks, and reliability issues in central components can easily affect the whole deployment. To address these challenges, we explore and adapt semi-decentralized training techniques for Spatio-Temporal Graph Neural Networks (ST-GNNs) in smart mobility domain. We implement a simulation framework where sensors are grouped by proximity into multiple cloudlets, each handling a subgraph of the traffic graph, fetching node features from other cloudlets to train its own local ST-GNN model, and exchanging model updates with other cloudlets to ensure consistency, enhancing scalability and removing reliance on a centralized aggregator. We perform extensive comparative evaluation of four different ST-GNN training setups---centralized, traditional FL, server-free FL, and Gossip Learning---on large-scale traffic datasets, the METR-LA and PeMS-BAY datasets, for short-, mid-, and long-term vehicle speed predictions. Experimental results show that semi-decentralized setups are comparable to centralized approaches in performance metrics, while offering advantages in terms of scalability and fault tolerance. In addition, we highlight often overlooked issues in existing literature for distributed ST-GNNs, such as the variation in model performance across different geographical areas due to region-specific traffic patterns, and the significant communication overhead and computational costs. However, due to planar nature of graphs, per-cloudlet costs remains consistent as the network grows, unlike the growing costs in a centralized approach.
% that arise from the large receptive field of GNNs, leading to substantial data transfers and increased computation of partial embeddings.
\end{abstract}

==> section_v2/1_introduction.tex <==
\section{Introduction}

\begin{figure*}[ht!]
  \centering
  \includegraphics[width=0.9\linewidth]{figures/intro-figure-row.png}
  \caption{Graph partitioning and communication. a) Geographically distributed sensor network and base stations b) Graph partitioning of the sensors into cloudlets based on geographical proximity. c) Cloudlet-to-cloudlet communication network for exchanging node features and model updates. d) After communicating with neighbouring cloudlets, each cloudlet can construct the ST-GNN subgraph required for training on its local nodes}
  \label{fig:0.5}
\end{figure*}

Smart mobility is integral to urban planning, particularly in transportation systems, influencing development and traffic management \cite{cite_1}. Traffic prediction is a key component of smart mobility \cite{cite_2, cite_3, cite_4, cite_5, cite_6} and includes tasks such as vehicle speed and public transport forecasting. As demand for these services rises, the need for accurate and efficient traffic forecasting grows, enabling effective resource management, congestion reduction, and route optimization.

% Smart mobility is a growing focus in urban planning, especially within transportation systems, where it influences both urban development and transport planning \cite{cite_1}. A key component of smart mobility is traffic prediction \cite{cite_2, cite_3, cite_4, cite_5, cite_6}, which includes tasks like predicting vehicle speeds and public transport usage. As demand for these services rises, the need for accurate and efficient traffic forecasting grows, enabling effective resource management, congestion reduction, and route optimization.

Like other prediction tasks, traffic forecasting methods can generally be divided into classical statistical methods like autoregressive integrated moving average (ARIMA) \cite{cite_34} and Deep Learning (DL)-based methods such as Long Short-Term Memory (LSTM) \cite{cite_7} and Diffusion Convolutional Recurrent Neural Networks (DCRNN) \cite{cite_8}. However, both approaches only use temporal dependencies, overlooking spatial ones.

% Like other prediction tasks, traffic forecasting methods can generally be divided into classical statistical approaches and Deep Learning (DL)-based approaches. In time-series analysis, autoregressive integrated moving average (ARIMA) and its variants are one of the most consolidated approaches based on classical statistics \cite{cite_34}, while for DL-based approaches they are Long Short-Term Memory (LSTM) \cite{cite_7} or Diffusion Convolutional Recurrent Neural Networks (DCRNN) \cite{cite_8}. However, both approaches only use temporal dependencies, overlooking spatial ones.

Graph Neural Networks (GNNs) \cite{cite_29} address these issues by modeling traffic data as a graph, where nodes represents a physical location, and edges spatial connections between these locations. Specifically, Spatio-Temporal Graph Neural Networks (ST-GNNs) \cite{cite_16} extend GNNs to capture both spatial and temporal dependencies, making them more effective than other DL-based approaches for traffic forecasting.  Thus, numerous ST-GNN architectures have been developed and tested for this task \cite{cite_16}.

% Numerous ST-GNNs have been developed, such as Graph Recurrent Network (GRN) \cite{cite_12}, Spatio-Temporal Graph Convolutional Network (ST-GCN) \cite{cite_13}, Graph Attention LSTM Network \cite{cite_14}, and many more \cite{cite_16}. Each technique addresses specific challenges or offers unique advantages over others. %In this work, ST-GCN will be used due to its superior ability to handle traffic prediction tasks compared to other techniques.

However, most previous works have focus on ST-GNN trained in centralized environments, where data from all sensors is continuously collected. But the task of collecting data, performing DL training and inference, and sending back commands is challenging to perform reliably in real-time in a centralized system. As sensors networks expand, scaling a central control system to handle the increased volume of data in real-time with low-latency becomes increasingly difficult. Furthermore, any issues in the central control system can easily result in a complete interruption of the service, requiring significant investments to maximize reliability. Given the key role played by mobility infrastructure in our societies, a centralized system can also become a significant target for hostile actors and a major cyber-weakness in strategic infrastructure management.

% However, most previous works have focused on ST-GNNs trained in centralized environments, where data from all sensors is continuously collected. But the task of collecting geo-distributed data, performing deep learning training and inference, and sending back commands (such as updating traffic light schedules based on predicted traffic patterns), is challenging to perform reliably in real-time in a centralized system. As sensors networks expand---either by covering larger, more distant regions or by increasing their density to provide more granular sensing in urban areas---scaling a central control system to handle the increased volume of data in real-time with low-latency becomes increasingly difficult. Furthermore, any issues in the central control system can easily result in a complete interruption of the service across the whole sensor network, requiring significant investments to maximize reliability. Given the key role played by mobility infrastructure in our societies, a centralized system can also become a significant target for hostile actors and a major cyber-weakness in strategic infrastructure management.

% However, the aforementioned approaches are predominantly designed for centralized environments, where data from distributed sources is collected and processed in a central server. As cities generate vast amounts of real-time traffic data, centralized data collection and processing struggles to keep pace with the ever-increasing data volume, leading to scalability and reliability issues. While traditional FL partially addresses the problem of centralized training, it still relies on a central aggregator to combine local models created by FL clients, and therefore cannot completely eliminate the aforementioned issues.

In this paper, we explore and adapt distributed training techniques for ST-GNNs in the smart mobility domain through semi-decentralized methods at the network edge, ensuring scalability and reliability. This approach utilizes geographically distributed cloudlets, hosted on edge devices with moderate computation and communication capabilities, as shown in Figure~\ref{fig:0.5}-a. Each cloudlet manages a subgraph of the overall traffic graph (Fig. \ref{fig:0.5}-b), shares node features necessary for local training step and model updates with other cloudlets to maintain consistency (Fig. \ref{fig:0.5}-c), and constructs ST-GNN subgraph required for training on its local nodes (Fig. \ref{fig:0.5}-d). The contributions of this paper can be summarized as follows:

\begin{itemize}
\item To our knowledge, we are the first to investigate semi-decentralize ST-GNN training with geographically distributed cloudlets
\item We develop a simulation framework for semi-decentralized ST-GNN training across cloudlets, allowing us to test different approaches.
\item Using our framework, we implement and compare four different training approaches---centralized, traditional FL, server-free FL, and Gossip Learning---providing the first comprehensive analysis of the benefits and drawback of these approaches for our targeted use-case, assessing their suitability for real-world deployment and informing future research endeavours.
\item We evaluate these approaches on two real-world datasets, METR-LA and PeMS-BAY \cite{cite_31}, across short-, mid-, and long-term traffic predictions, with a detailed analysis of model performance, cloudlet-specific metrics, communication overhead and computational costs.
\end{itemize}

Our experiments show that semi-decentralized approaches perform competitively against the centralized approach, especially for short-term prediction. Crucially, we provide insights on notable challenges in distributed ST-GNN training, which to our knowledge has not been explored in existing literature, such as highlighting the variation in model performance across different geographical areas due to region-specific traffic patterns, and the significant communication overhead and computational costs that arise from the large receptive field of GNNs, leading to substantial data transfers and increased computation of partial embeddings. However, communication overhead is mitigated by the planar structure of graphs, keeping per-cloudlet costs consistent as the network grows.

% our analysis highlights the variation in model performance across different geographical areas due to region-specific traffic patterns, and the significant communication overhead and computational costs that arise from the large receptive field of GNNs, leading to substantial data transfers and increased computation of partial embeddings. This insight sheds light on a notable challenges in distributed ST-GNN training, which to our knowledge has not been explored in existing literature.

% we are defining a scenario and a setup of a semi-dec env
% we are implementing a framework to test diferent approaches for distributed training in our scenario
% we perform extenstive experiments(analysis) with the goal of comparing different training setups and highlight the tradeoffs that's often missed in existing literature (on this very relevant topic that's not been explored that much)

==> section_v2/2_preliminaries.tex <==
\section{Preliminaries}\label{sec:preliminares}
\subsection{Traffic prediction}
Traffic prediction is one of the most common and critical time-series forecasting tasks, as it estimates traffic metrics, such as speed, volume, and density to monitor current traffic conditions and predict future trends. It is generally classified into three forecasting horizons: short-term (15 min), mid-term (30 min), and long-term (60 min). In the context of ST-GNNs, the traffic system is represented as a spatial graph at the \textit{t}-th time step, denoted by $\mathcal{G}_t$ = ($\mathcal{V}_t$, $\mathcal{E}$, W), where $v_i, v_j\in \mathcal{V}_t$ is a finite set of nodes corresponding to observations from \textit{n} IoT-devices in the traffic network, $(v_i, v_j)\in \mathcal{E}$ is a set of edges connecting the IoT-devices, and $W\in \mathbb{R}^{n \times n}$ is a weighted adjacency matrix that encodes the spatial relationships between these IoT-devices. The spatial component is defined by the physical locations of IoT devices, while the temporal component arises from traffic features that evolve over time, influencing the graph's dynamics. While this work focuses on traffic prediction, methods for other smart mobility tasks can be generalized to this domain due to their shared reliance on spatio-temporal data. 

\subsection{Spatio-Temporal Graph Neural Networks}
ST-GNNs are DL models designed to capture both spatial and temporal dependencies in structured data, allowing it to simultaneously account for spatial correlations between nodes and temporal correlations over time, making it particularly suited for traffic prediction. By leveraging spatial dependencies, ST-GNNs provide a more accurate representation of how local traffic conditions at one location impact neighbouring locations.

Multiple ST-GNNs have been developed \cite{cite_16}, such as Graph Recurrent Network (GRN) \cite{cite_12}, Spatio-Temporal Graph Convolutional Network (ST-GCN) \cite{cite_13}, Graph Attention LSTM Network \cite{cite_14}, and many more \cite{cite_16}. Each technique addresses specific challenges or offers unique advantages over others. In this paper, we utilize ST-GCN due to their superior ability to handle traffic prediction tasks in the IoT context compared to other techniques. Experiments demonstrated that ST-GCN consistently outperforms other models in key evaluation metrics (MAE, MAPE, and RMSE) \cite{cite_13}.

\subsection{Traditional Federated Learning}
Traditional FL \cite{cite_30} is a collaborative machine learning (ML) approach where multiple clients work together to train a model, coordinated by a central aggregator. Instead of sharing raw data, which remains stored locally on each client device, the clients exchange only model updates with the server. These updates contain just the minimum information needed for the learning task, carefully scoped to limit the exposure of client data. The central aggregator then aggregates these focused updates as soon as they are received, ensuring that the learning process is both efficient and compliant with data minimization principles.

\subsection{Server-free Federated Learning}
Server-free FL \cite{cite_26} is a decentralized variant of the traditional FL approach. Unlike traditional FL, where a central aggregator is responsible for coordinating the model updates, server-free FL operates without a central entity. Instead, participating devices communicate directly with one another to exchange model parameters and perform local updates. After initializing their models, devices exchange model parameters with their neighbours, aggregate these received models with their own local model, and proceed to train on a subset of data. This iterative process allows for continuous refinement of models across the network, as the updated models are exchanged again between neighbouring devices.


\subsection{Gossip Learning}
Gossip Learning \cite{cite_27} is a decentralized protocol for training ML models in distributed settings without the need for a central coordinator. It is designed to be highly scalable and robust, allowing model updates to be propagated efficiently across a network of devices or nodes. Each device stores two models in its memory (as a FIFO buffer), typically representing the most recent models received from neighbouring devices. At each iteration of the gossip protocol, a device averages the weights of these two models to create an aggregated model. The device then performs one local training step using its own data, refining the aggregated model based on its local observations. Once the model is updated, the device forwards it to a randomly chosen device in the entire network. This process is repeated across the network, ensuring that models continuously evolve and improve as they traverse different nodes, collecting knowledge from the data they encounter at each location.

==> section_v2/3_methodology.tex <==
\section{Methodology}
\subsection{Scenario}
The traffic prediction scenario involves IoT-devices (i.e., sensors) deployed along highways to monitor real-time traffic conditions such as vehicle speed, volume, and density at fixed time intervals. To streamline data processing, IoT-devices are assigned to local base stations (BS), referred to as cloudlets, based on their physical proximity and communication range. The communication between IoT-devices and its BS is facilitated using Low-Power Wide-Area Network (LPWAN) protocols, such as LoRa or NB-IoT, which enable efficient, long-range, and low-power data transmission. Base stations, in addition to serving as communication hubs, are equipped with moderate computational resources. This existing computational power can be leveraged for training ML models, such as ST-GNNs. % By utilizing this infrastructure, the system reduces dependency on centralized servers, enabling localized model training and real-time traffic analysis while enhancing scalability and eliminating single points of failure.

\subsection{Distributed Training Setups}
We adopt a semi-decentralized ST-GNN architecture inspired by Nazzal et al. \cite{cite_25}, as it's one of the most effective architectures for distributed training. Figure~\ref{fig:0.5} shows key components of such architecture. In Fig.~\ref{fig:0.5}-a, traffic network is represented as a graph, where nodes correspond to IoT-devices, and edges represent road connections based on physical proximity. In Fig.~\ref{fig:0.5}-b, the graph is partitioned into subgraphs based on geographical proximity, each managed by a local cloudlet. In Fig.~\ref{fig:0.5}-c, cloudlets form a communication network for exchanging necessary node features and model updates. After communicating with each other, each cloudlet constructs ST-GNN subgraph required for training on its local nodes, as shown in Fig.~\ref{fig:0.5}-d.

% talk 1st about figure 1 and then the approaches (setups)
Using this architecture, we evaluate four different training setups---centralized, traditional FL, server-free FL, and Gossip Learning---for ST-GNNs in the context of traffic prediction, with the centralized setup serving as a baseline for comparing the semi-decentralized approaches.

% In the traditional FL setup, we use a central aggregator to form a global model shared across cloudlets, while in server-free FL cloudlets communicate directly with their neighboring cloudlets to exchange and aggregate model updates. As for Gossip Learning, cloudlets iteratively exchange and update models with randomly selected peers. Each setup is evaluated in terms of communication, computation, and prediction performance.

\subsection{GNN Partitioning in Distributed Training}
Partitioning the graph into subgraphs for local training in distributed GNN scenarios presents unique challenges due to their reliance on spatial dependencies. Unlike traditional ML models that process localized data independently, GNNs require information from neighbouring nodes to compute effective representations. Specifically, in an $\ell$-layer GNN, the representation of a node depends not only on its own features but also on the features of its $\ell$-hop neighbours.
% Partitioning the graph into subgraphs for local training in distributed scenarios presents unique challenges for Graph Neural Networks (GNNs) due to their reliance on spatial dependencies. Unlike traditional ML models that process localized data independently, GNNs require information from neighbouring nodes to compute effective representations. Specifically, in an $\ell$-layer GNN, the representation of a node depends not only on its own features but also on the features of its $\ell$-hop neighbours.

This spatial dependency introduces a need for inter-cloudlet communication, as the required node features often extend beyond the boundaries of a single cloudlet's subgraph. Since IoT-devices typically have limited communication capabilities and cannot directly exchange data with distant cloudlets, the necessary node features are shared between the cloudlets themselves.

Each cloudlet, based on the underlying sensor network connectivity, is aware of which neighbouring cloudlets require its node features for local computations. When features are collected from the IoT-sensors, the cloudlet proactively broadcasts these features to the neighbouring cloudlets that need them for training (Fig.~\ref{fig:0.5}-d). This proactive exchange of node features ensures that each cloudlet has sufficient information to perform local computations without compromising the accuracy of the GNN model.
% In distributed training scenarios involving GNNs, partitioning the graph into subgraphs for local training introduces unique challenges due to the spatial dependencies inherent in GNN architectures. Unlike traditional ML models that operate independently on localized data, GNNs require access to information from neighboring nodes to perform effective computations. Specifically, for an $\ell$-layer GNN, each node's representation depends not only on its own features but also on the features of its $\ell$-hop neighbors. This dependency extends beyond the immediate boundaries of a cloudlet’s partitioned subgraph, requiring inter-cloudlet communication to exchange node features. To address this challenge, our framework ensures that each cloudlet collects not only the data from its directly assigned IoT-devices but also the node features of neighboring nodes located in other partitions. 

==> section_v2/4_experimental_setup.tex <==
\section{Experimental Setup}
\subsection{Datasets}
To evaluate the performance of our setups, we utilize two real-world public traffic datasets, PeMS-BAY\footnote{\label{footnote_1}Download link: \url{https://github.com/liyaguang/DCRNN}} and METR-LA\footref{footnote_1} \cite{cite_31}, which are collected by Caltrans performance measurement system. Both datasets consist of traffic data aggregated in 5-minute intervals, with each sensor collecting 288 data points per day. The details of datasets are listed in Table~\ref{table:1}.

% TABLE I
\begin{table}[htbp]
    \centering
    \caption{Details of METR-LA and PeMS-BAY}
    \begin{tabular}{c c c c c}
        \hline
        Datasets & Nodes & Interval & TimeSteps & Attribute \\
        \hline
        METR-LA & 207 & 5 min & 34,272 & Traffic speed \\
        PeMS-BAY & 325 & 5 min & 52,116 & Traffic speed \\
        \hline
    \end{tabular}
    \label{table:1}
\end{table}

The spatial adjacency matrix is constructed from the actual road network based on distance using the formula from ChebNet \cite{cite_28}. Specifically, it encodes the spatial relationships between nodes by assigning weights to edges based on the inverse of the pairwise distances between connected nodes, effectively capturing the connectivity and proximity of locations in the traffic network. Additionally, the data were preprocessed for efficient model training and evaluation. For example, if we want to utilize the historical data spanning one hour to predict the data the next hour, we pack the sequence data in group of 12 and convert it into an instance. The dataset was then split into training, validation, and test sets in a 70:15:15 ratio. Additionally, to mitigate the impact of varying data magnitudes, we applied standardization to normalize the original data values, reducing the impact of the large difference in value.

\begin{comment}
\subsection{Model Architecture}
We adopt a semi-decentralized architecture utilizing local cloudlets, each handling a subgraph of the traffic graph, inspired by the approach proposed by Nazzal et al. \cite{cite_25}, as it's one of the most effective architectures for distributed training. Figure~\ref{fig:0.5} 

By focusing on this architecture, our framework is able to leverage the strengths of semi-decentralized approaches, effectively combining localized computation with inter-cloudlet collaboration. This design enables efficient distributed training of ST-GNNs while addressing challenges such as limited local input access and the need for scalable communication. As shown in Fig.~\ref{fig:1}, cloudlets form a semi-decentralized architecture where:

\begin{itemize}
\item IoT-devices send traffic data to their cloudlet;
\item Cloudlets train local ST-GNN models on the received data, capturing both the spatial and temporal patterns of the traffic;
\item Cloudlets send node features of its IoT-devices to other cloudlets for local training purposes; and 
\item Cloudlets communicate with other cloudlets to exchange model updates in decentralized scenarios such as server-free FL and gossip learning.
\end{itemize}
\end{comment}

\subsection{Evaluation Metrics}
In our experiments, we evaluate the performance of different setups using Weighted Mean Absolute Percentage Error (WMAPE), in addition to the widely adopted Mean Absolute Error (MAE) and Root Mean Square Error (RMSE). We use WMAPE because it accounts for the varying magnitudes of traffic speeds across regions, providing a more balanced evaluation. We omit the formulas for MAE and RMSE due to their wide adoption. The WMAPE formula is as follows:

\begin{equation}
    \text{WMAPE}(\bm{x}, \bm{\hat{x}}) = \frac{\sum_{i}{\mid x_i - \hat{x}_i \mid}}{\sum_{i}{\hat{x}_i}} * 100\%,
\end{equation}

\noindent where $\bm{x} = x_1,\ldots,x_n$ denotes the ground truth values of vehicle speed, and $\bm{\hat{x}} = \hat{x}_1,\ldots,\hat{x}_n$ represents their predicted values.

We compute these metrics across three forecasting horizons—--short-, mid-, and long-term---to capture fluctuations in performance over time. For centralized and FL setups, the metrics are derived from the main server's aggregated model, while for server-free FL and Gossip Learning, they are computed as a weighted average of the individual cloudlet predictions. This ensures a consistent and fair comparison across all approaches.

% Figure 2
\begin{figure}[h]
  \centering
  \includegraphics[width=0.9\linewidth]{figures/locations_metr-la_pems-bay_experiment_1_subplot.png}
  \caption{Sensor assignment to cloudlets based on communication range}
  \label{fig:2}
\end{figure}

\subsection{Experimental Setup}
% TABLE II
\begin{table*}[ht!]
\centering
\caption{Performance Comparison (MAE [$mile/h$]/RMSE [$mile/h$]/WMAPE [\%]) of four different setups}
\label{table:2}
\renewcommand{\arraystretch}{1.5} % Adjust row spacing for better readability
\begin{tabular}{l l ccc | ccc | ccc}
\hline\hline
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Setups} & \multicolumn{3}{c|}{15 min} & \multicolumn{3}{c|}{30 min} & \multicolumn{3}{c}{60 min} \\ 
\cline{3-11}
\multicolumn{2}{l}{} & MAE & RMSE & WMAPE & MAE & RMSE & WMAPE & MAE & RMSE & WMAPE \\ 
\hline\hline
\multirow{4}{*}{METR-LA} & Centralized             & 3.78 & 9.05      & 7.45 & 5.14 & 11.61       & 10.12 & 7.35 & 14.59      & 14.47 \\ \cline{3-11}
                                      & Traditional FL      & 3.97 & 9.01       & 7.82 & 5.40 & 11.41       & 10.63 & 7.82 & 14.48      & 15.40 \\ \cline{3-11}
                                      & Server-free FL          & 3.90 & 8.98 & 7.78     & 5.35 & 11.37 & 10.67     & 7.79 & 14.41 & 15.55 \\ \cline{3-11}
                                      & Gossip Learning         & 3.88 & 9.04 & 7.74     & 5.43 & 11.35 & 10.85     & 7.56 & 14.42 & 15.10 \\ 
\hline\hline
\multirow{4}{*}{PeMS-BAY} & Centralized             & 1.48 & 3.09      & 2.38 & 1.97 & 4.23      & 3.17 & 2.59 & 5.41      & 4.17 \\ \cline{3-11}
                                       & Traditional FL      & 1.50 & 3.12      & 2.42 & 2.03 & 4.29      & 3.27 & 2.67 & 5.51      & 4.29 \\ \cline{3-11}
                                       & Server-free FL          & 1.50 & 3.12 & 2.42    & 2.01 & 4.25 & 3.23      & 2.65 & 5.44 & 4.28 \\ \cline{3-11}
                                       & Gossip Learning         & 1.51 & 3.12 & 2.43    & 2.03 & 4.28 & 3.26      & 2.63 & 5.39 & 4.24 \\ 
\hline\hline
\end{tabular}
\end{table*}

All experiments were run with a fixed number of 40 epochs, utilizing the High-Performance Computing (HPC) system Leonardo Booster, which features 4x NVIDIA A100 SXM6 64GB GPUs, with only 1 being used during training. The software environment used for the experiments included Python 3.10.14, PyTorch 2.3.1, and PyTorch Geometric 2.5.3.

For model architecture, we used 2 spatio-temporal blocks (ST-blocks), with GLU activation function, a learning rate of 0.0001, dropout of 0.5, weight decay of 0.00001, and a batch size of 32. MAE is used as the training loss, Adam was chosen as the optimization algorithm, and learning rate scheduler was applied with the StepLR strategy, where the step size was set to 5, and the decay factor was set to 0.7. The temporal and spatial kernel size was set to 3 for all experiments, with Chebyshev convolution as convolutional layer. All experiments use 60 minutes as the historical time window, i.e., 12 observed data points.

Additionally, sensors were distributed across 7 cloudlets based on proximity and communication range. While algorithms such as k-means clustering could have been used to distribute sensors to cloudlets, we manually defined cloudlet placement to ensure full coverage of the geographical area in each dataset. Each cloudlet can communicate with other cloudlets and IoT-devices only if they are within an 8 km range. This limitation directly impacts the server-free FL approach by restricting the number of cloudlets that can exchange model updates. In contrast, this constraint does not affect Gossip Learning, as model updates are sent to a randomly selected cloudlet across the entire network, regardless of proximity. Fig.~\ref{fig:2} shows how sensors are assigned to cloudlets and their respective communication ranges for both the METR-LA and PeMS-BAY datasets. This partitioning reflects the semi-decentralized structure used for our distributed training approach.

==> section_v2/5_experimental_results.tex <==
\section{Experimental Results}
\subsection{Comparison of training setups}
Table~\ref{table:2} presents the results of all setups, datasets, and forecast horizons. Centralized training consistently outperforms semi-decentralized methods across all metrics and horizons. However, the performance gap is minimal, especially for MAE and RMSE. For instance, in the METR-LA dataset, the MAE difference between centralized and the best semi-decentralized setup is only 0.1 mph for short-term predictions—negligible compared to typical traffic flow variations, often measured in tens of mph. While WMAPE shows a slightly larger gap as the forecast horizon increases, particularly for METR-LA, the difference remains narrow across all horizons. This indicates that semi-decentralized setups offer competitive performance with no significant practical drawbacks for traffic prediction.
% Table~\ref{table:2} presents the results of four training setups, across both datasets for three forecast horizons. The table  highlights that the centralized setup consistently outperforms the semi-decentralized methods across all evaluation metrics and forecast horizons. The observed performance gap is extremely small between all 4 setups, especially for MAE and RMSE. For example, in the METR-LA dataset, the difference in MAE between the centralized setup and the best semi-decentralized setup is 0.1 miles per hour for short-term prediction, which is negligible compared to the difference between normal traffic flow and a traffic jam, typically measured in tens of miles per hour. While WMAPE shows a slightly more noticeable gap as the forecast horizon increases, particularly for the METR-LA dataset, the difference between centralized and semi-decentralized methods remains within a narrow margin across all horizons. In other words, this difference is insignificant to disregard the competitive performance of semi-decentralized approaches compared to the centralized one, indicating no practical drawbacks in adopting semi-decentralized methods for traffic prediction use-case.

\subsection{Cloudlet Metric Analysis}
% Figure 3
\begin{figure*}[ht!]
  \centering
  \includegraphics[width=0.85\linewidth]{figures/plot_val_metric_WMAPE_metr-la_pems-bay_cloudlet_subplot.png}
  \caption{WMAPE for individual cloudlets}
  \label{fig:3}
\end{figure*}

Figure~\ref{fig:3} shows WMAPE variability across cloudlets for all setups and datasets, focusing on short- and long-term predictions, providing a comprehensive view of how errors distribute geographically across cloudlets for different prediction horizons. WMAPE is highlighted as it provides a clear, percentage-based measure of relative error, making it easier to compare variability across cloudlets. 

% Figure~\ref{fig:3} illustrates the variability in WMAPE across individual cloudlets for all training setups and both datasets. The results are shown for short-term and long-term prediction horizons, providing a comprehensive view of how errors distribute geographically across cloudlets for different prediction horizons. We focus exclusively on WMAPE because all metrics exhibit similar patterns of spread across cloudlets. However, WMAPE is particularly insightful as it highlights the relative error in percentage terms, making it easier to interpret and compare the variability across different cloudlets.

The figure reveals consistent WMAPE spread across cloudlets, regardless of training setup, dataset, or horizon, indicating that performance variability stems from the datasets' geographical characteristics and sensor partitioning, rather than the training methods. Each cloudlet's performance is influenced by the distribution of sensors assigned to it and the corresponding traffic patterns in that geographical region.

% From the figure, we observe consistent spread in WMAPE values across cloudlets, irrespective of the training setup, dataset, or prediction horizon. This consistency suggests that the variability in cloudlet performance is not an artifact of the training setups, but is instead intrinsic to the geographical characteristics of the datasets and sensor partitioning, alongside the values of data itself. Each cloudlet's performance is influenced by the distribution of sensors assigned to it and the corresponding traffic patterns in that geographical region.

Additionally, while global weighted averages reported in Table~\ref{table:2} provide a summary of performance, they fail to capture the significant differences in performance across individual cloudlets. Previous works have primarily focused on global averages, overlooking notable challenge of heterogeneous performance among cloudlets. This oversight can lead to an incomplete understanding of model performance in distributed traffic forecasting systems, resulting in unexpected discrepancies, suboptimal decision-making and potential disruptions in real-world usage compared to testing.
% Figure 4
\begin{figure}[h]
  \centering
  \includegraphics[width=0.9\linewidth]{figures/plot_val_loss_metr-la_pems-bay_multi_subplot.png}
  \caption{Validation loss over FLOPs and epochs for short-term prediction}
  \label{fig:4}
\end{figure}

% TABLE III
\begin{table*}[htbp]
    \centering
    \caption{FLOPs and average model and node feature transfer size}
    \label{table:3}
    \renewcommand{\arraystretch}{1.5} % Adjust row spacing for better readability
    \begin{tabular}{l l c | c | c | c}
    \hline\hline
    \multirow{1}{*}{Dataset} & \multirow{1}{*}{Setups} & \multicolumn{1}{c|}{Model [MB]/epoch} & \multicolumn{1}{c|}{Training FLOPs/epoch} & \multicolumn{1}{c|}{Aggregation FLOPs/epoch} & \multicolumn{1}{c}{Node feature [MB]}\\ 
    % Header row
    %\multicolumn{2}{l}{} & Model [MB] & Node feature [MB] \\ 
    \hline\hline
    % METR-LA rows
    \multirow{4}{*}{METR-LA} 
        & Centralized              & - & 1.68T & - & 4.76 \\ \cline{3-6}
        & Traditional FL & 0.91 / 7 & 10.92T / 7 & 1.12M / 7 & 25.83 / 7 \\ \cline{3-6}
        & Server-free FL           & 1.61 / 7 & 10.92T / 7 & 3.64M / 7 & 25.83 / 7 \\ \cline{3-6}
        & Gossip Learning          & 0.91 / 7 & 10.92T / 7 & 2.94M / 7 & 25.83 / 7 \\ 
    \hline\hline
    % PeMS-BAY rows
    \multirow{4}{*}{PeMS-BAY} 
        & Centralized              & - & 4.06T & - & 11.27 \\ \cline{3-6}
        & Traditional FL & 0.91 / 7 & 27.23T / 7 & 1.12M / 7 & 66.08 / 7 \\ \cline{3-6}
        & Server-free FL           & 1.82 / 7 & 27.23T / 7 & 3.92M / 7 & 66.08 / 7 \\ \cline{3-6}
        & Gossip Learning          & 0.91 / 7 & 27.23T / 7 & 2.94M / 7 & 66.08 / 7 \\ 
    \hline\hline
    \end{tabular}
\end{table*}

\subsection{Analysis of semi-decentralized overheads}
Semi-decentralized learning naturally introduces several overheads, primarily stemming from the need to communicate and aggregate models, increasing communication and computational costs compared to centralized training. Additionally, due to graph partitioning, node features must be exchanged between cloudlets, further contributing to communication and compute demands. Table~\ref{table:3} breaks down these overheads across three key aspects: model transfer, node feature transfer, and floating-point operations (FLOPs).

A significant communication cost arises from node feature transfers. Unlike centralized training, where each sensor's features are sent once to a central server, distributed setups require sending features to multiple cloudlets. This increase is due to the dense graph created by our distance-based weighted adjacency matrix and the 2-hop GNN, which requires each cloudlet to process features from both direct and indirect neighbors. Consequently, each cloudlet processes a substantial graph portion, leading to several-fold higher communication costs compared to centralized setups. However, as the network grows larger, the portion of the graph stored in each cloudlet will decrease, as cloudlets farther away will not have connected sensors. Despite the increase, the overall feature transfer per cloudlet remains manageable, typically just a few megabytes.

% One of the most significant communication costs in semi-decentralized training is the transfer of node features. Unlike centralized training, where each sensor's features are sent once to a central server, distributed setups require features to be transferred to potentially multiple cloudlets. This increase is due to our distance-based weighted adjacency matrix creating a relatively dense graph, where each sensor node is connected to all other nodes within a predefined radius, and the use of a 2-hop GNN, meaning that each cloudlet not only needs features from its direct neighbours but also from the neighbours of those neighbours, significantly expanding the portion of the graph that each cloudlet must process. Consequently, each cloudlet must store and process a substantial portion of the entire graph, leading to a several-fold increase in communication compared to centralized setups. However, as the network grows larger, the portion of the graph stored in each cloudlet will decrease, as cloudlets farther away will not have connected sensors. Despite the increase, the overall feature transfer per cloudlet remains manageable, typically just a few megabytes.

In contrast, model transfer per epoch is relatively small due to the compact size of ST-GCN models. While model transfers accumulate over time, contributing to total communication overhead, the per-epoch cost remains in the order of megabytes. As shown in Figure~\ref{fig:4}, distributed setups, particularly server-free FL, require more epochs to converge than centralized training, increasing total model transfer costs. Despite this, even in server-free FL’s worst-case scenario, where all cloudlets communicate with each other, model transfer remains a minor overhead.

% In contrast to node feature transfers, model transfer per epoch remains relatively small across all distributed setups. This is primarily due to the compact size of the ST-GCN models used in our experiments. While model transfers accumulate over multiple epochs, leading to higher total communication overhead, the per-epoch cost remains in the order of megabytes. As shown in Figure~\ref{fig:4}, distributed setups, particularly server-free FL, require more epochs to converge than centralized training, compounding the total model transfer cost. Despite this, the overall communication overhead from model transfers remains modest and does not present a significant bottleneck. Even in the worst-case scenario of server-free FL, where all cloudlets potentially communicate with each other, the model transfer overhead remains manageable.

Computation-wise, aggregation costs are many orders of magnitude smaller training costs, so they do not represent a reason to avoid semi-decentralized training. However, distributed setups incur significantly higher training costs than centralized ones, mirroring the feature transfer pattern. Each cloudlet runs the model on its local subgraph, often with duplicated nodes and features due to overlapping receptive fields. This duplication results in additional computations, as cloudlets must compute partial embeddings for nodes they do not own. In contrast, centralized training efficiently processes the entire graph without redundancies, avoiding duplicated calculations.

% In terms of computation, we see that aggregation costs are many orders of magnitude smaller than training costs, so they do not represent a reason to avoid semi-decentralized training. In contrast, the training costs in distributed setups are several times higher than in centralized training. This mirrors the pattern observed in feature transfer, as the root cause is similar. Each cloudlet must run the GNN on its local subgraph, which often includes duplicated nodes and features due to the overlapping receptive fields of neighbouring cloudlets. This duplication leads to additional computations, as cloudlets must compute partial embeddings for nodes they do not own to facilitate GNN message passing within their local subgraph. Only the cloudlet that owns a node can compute its full k-hop embedding and make accurate predictions. In contrast, a centralized system can efficiently train over the entire graph without such redundancies, avoiding duplicated computations.

Our analysis shows that the primary overheads in semi-decentralized training stem not from the distributed learning algorithms themselves, but from the highly interconnected spatial nature of traffic data and the need to partition these spatial connections across cloudlets. If these algorithms were applied to non-spatial models, the overheads would be minimal. While communication and computation costs are higher than in centralized setups, they remain within acceptable limits, making semi-decentralized training a practical solution for scalable traffic prediction in smart mobility applications.

% Our analysis reveals that the major sources of overhead in semi-decentralized training do not stem from the distributed learning algorithms themselves. If these algorithms were applied to non-spatial models, the overheads would be minimal. Instead, the overheads arise from the highly interconnected spatial nature of traffic data and the need to partition these spatial connections across cloudlets. Overall, the trade-off between the flexibility and scalability of semi-decentralized training and the increased communication and computational overheads highlights the challenges of maintaining spatial dependencies in distributed setups. While the communication and computation costs are higher than centralized training, they remain within acceptable limits, making semi-decentralized approaches a feasible solution for scalable traffic prediction in smart mobility applications.

% Table~\ref{table:3} breaks down these overheads across three key aspects: model transfer, node feature transfer, and floating-point operations (FLOPs). The table shows that the computational cost of aggregation in traditional FL is negligible compared to the overall training cost, making the central aggregator less critical. Instead of central aggregator, aggregation can be performed locally on each cloudlet with minimal impact on performance. Additionally, the table shows that model transfer size varies between setups, reflecting the difference in communication patterns. Theoretically, for server-free FL, the model transfer size could be as large as $cln\_num * (cln\_num - 1) * Model [MB]$ if every cloudlet communicated with every other cloudlet in the network. However, due to the limited communication range of cloudlets, this theoretical upper bound is not reached. Despite that, model transfer size is relatively small compared to node feature transfers. This is due to graph connectivity being based on physical proximity rather than actual road networks, and the receptive field of GNNs expanding with each additional layer, necessitating the transfer of more node feature data across cloudlets \cite{cite_32} and increased computation of partial embeddings during training. As a result, node features contribute significantly to both communication overhead and computational cost.

% As seen in Figure~\ref{fig:4}, distributed setups converge with slightly more epochs compared to centralized, resulting in additional model transfers during the training process. Furthermore, due to extensive node feature transfers and additional local processing, the figure shows that distributed setups require significantly more computational power to converge compared to centralized training. This highlights the trade-off between the flexibility and scalability of semi-decentralized training and the increased communication overhead, computational costs and model transfer frequency required to reach convergence.


==> section_v2/6_related_work.tex <==
\section{Related Work}
Training and testing GNN models on large graphs demand substantial memory and processing resources due to the interdependence of graph nodes \cite{cite_17}. This creates a scalability and reliability issues for centralized GNN operations \cite{cite_18}, especially when dealing with large-scale graphs or sensitive data collected from distributed sensors in real-time traffic prediction.

\subsection{Centralized ST-GNN training}\label{AA}
However, the majority of existing approaches for training ST-GNNs are based on centralized architectures \cite{cite_12, cite_13, cite_14, cite_15}. While this approach allows for the direct management of both spatial and temporal correlations, ensuring that the full context of the data can be leveraged to improve the models accuracy and performance, it comes with significant limitations as described above.

\subsection{Traditional Federated Learning ST-GNN training}\label{AA}
Several works have applied traditional FL to train ST-GNN models for traffic prediction \cite{cite_20, cite_21, cite_22, cite_23}. One of the primary advantages of traditional FL is enhanced scalability. By distributing the training process, it leverages the computational resources of multiple devices, which allows larger datasets to be processed without overloading any single server. While this approach improves on centralized training, it still relies on a central aggregator, meaning that it shares the same issues as centralized approach, as was already described above.

\subsection{Decentralized and semi-decentralized ST-GNN training}
To the best of our knowledge, there has been no prior research specifically focused on decentralized or even semi-decentralized training of ST-GNNs for traffic prediction.

One relevant work by L. Giaretta et. al. \cite{cite_24} explores the challenges and solutions associated with fully decentralized training. However, their solution is not tailored to ST-GNNs, but rather to Graph Convolutional Network (GCN), limiting its applicability to traffic prediction tasks that require both spatial and temporal correlations.

While there is no prior research work for decentralized training for ST-GNNs, M. Nazzal et. al. \cite{cite_25} developed Heterogeneous Graph Neural Network with LSTM (HetGNN-LSTM) for taxi-demand prediction and tested it in a semi-decentralized environment, where nodes were partitioned into cloudlets, without any central aggregator. However, their solution only enables semi-decentralized inference by deploying a pre-existing model, with no support for semi-decentralized training.

==> section_v2/7_future_work.tex <==
\section{Future Work}
\subsection{Communication and computation overhead}
Future work should address the significant communication overhead arising from node feature transfers, which dominate the bandwidth in semi-decentralized training, and increased computation of partial embeddings during training. While communication is feasible in these setups, the cost is significant compared to centralized training. Future work should aim to shift the trade-off between scalability and reliability by reducing both network overhead and computational cost without compromising model accuracy by exploring these directions:

\begin{itemize}
    \item Changing the network connectivity to be more sparse, replacing distance-based node connectivity with road network-based connectivity, with minimal impact on the model accuracy
    \item Restricting the receptive field of GNNs by adopting layer-wise GNN training, where the receptive field is constrained to avoid unnecessary feature propagation, as proposed by L. Giaretta et. al. \cite{cite_24}.
\end{itemize}

\subsection{Cloudlet personalization}
Another promising direction is implementing individual cloudlet personalization to address performance variability across cloudlets. Our results have highlighted a notable gap in error rates, especially in certain cloudlets with consistently higher error values. Personalizing cloudlets that have lower performance compared to the rest of the cloudlets, tailoring them to local traffic conditions or unique spatial-temporal patterns, could help reduce these disparities. Such a personalized approach may involve adjusting model parameters or incorporating local fine-tuning for cloudlets with higher error rates, potentially enhancing prediction accuracy across the network while maintaining decentralized resilience.

==> section_v2/8_conclusion.tex <==
\section{Conclusion}
In this paper, we have explored semi-decentralized approaches for traffic prediction in the smart mobility domain, comparing centralized, traditional FL, server-free FL, and Gossip Learning setups. By distributing ST-GNN training across multiple cloudlets, we aimed to address scalability and resilience challenges associated with traditional centralized approaches.

Experimental results on the METR-LA and PeMS-BAY dataset show that semi-decentralized setups are comparable to centralized approaches in performance metrics, while offering advantages in terms of scalability and fault tolerance. We also highlight often overlooked issues in existing literature for distributed ST-GNNs, such as the variation in model performance across different geographical areas due to region-specific traffic patterns, and the significant communication overhead and computational costs that arise from the large receptive field of GNNs, leading to substantial data transfers and increased computation of partial embeddings. However, due to the planar nature of graphs, cloudlets costs remains fixed as the network grows, unlike the growing costs in a centralized approach.

% We also highlight the often overlooked issues in existing literature, such as consistent spread in metric values across cloudlets, as well as dominant communication overhead and computational cost caused by node feature transfers and the amount of node features needed to be processed during training in distributed ST-GNNs.

==> section_v3/0_abstract.tex <==
\begin{abstract}
In smart mobility, large networks of geographically distributed sensors produce vast amounts of high-frequency spatio-temporal data that must be processed in real time to avoid major disruptions. Traditional centralized approaches are increasingly unsuitable to this task, as they struggle to scale with expanding sensor networks, and reliability issues in central components can easily affect the whole deployment. To address these challenges, we explore and adapt semi-decentralized training techniques for Spatio-Temporal Graph Neural Networks (ST-GNNs) in smart mobility domain. We implement a simulation framework where sensors are grouped by proximity into multiple cloudlets, each handling a subgraph of the traffic graph, fetching node features from other cloudlets to train its own local ST-GNN model, and exchanging model updates with other cloudlets to ensure consistency, enhancing scalability and removing reliance on a centralized aggregator. We perform extensive comparative evaluation of four different ST-GNN training setups---centralized, traditional FL, server-free FL, and Gossip Learning---on large-scale traffic datasets, the METR-LA and PeMS-BAY datasets, for short-, mid-, and long-term vehicle speed predictions. Experimental results show that semi-decentralized setups are comparable to centralized approaches in performance metrics, while offering advantages in terms of scalability and fault tolerance. In addition, we highlight often overlooked issues in existing literature for distributed ST-GNNs, such as the variation in model performance across different geographical areas due to region-specific traffic patterns, and the significant communication overhead and computational costs that arise from the large receptive field of GNNs, leading to substantial data transfers and increased computation of partial embeddings.
\end{abstract}

==> section_v3/1_introduction.tex <==
\section{Introduction}

\begin{figure*}[ht!]
  \centering
  \includegraphics[width=1\linewidth]{figures/intro-figure-row.png}
  \caption{Graph partitioning and communication. a) Geographically distributed sensor network and base stations b) Graph partitioning of the sensors into cloudlets based on geographical proximity. c) Cloudlet-to-cloudlet communication network for exchanging node features and model updates. d) After communicating with neighbouring cloudlets, each cloudlet can construct the ST-GNN subgraph required for training on its local nodes}
  \label{fig:0.5}
\end{figure*}

Smart mobility is integral to urban planning, particularly in transportation systems, influencing development and traffic management \cite{cite_1}. Traffic prediction is a key component of smart mobility \cite{cite_2, cite_3, cite_4, cite_5, cite_6} and includes tasks such as vehicle speed and public transport forecasting. As demand for these services rises, the need for accurate and efficient traffic forecasting grows, enabling effective resource management, congestion reduction, and route optimization.

Like other prediction tasks, traffic forecasting methods can generally be divided into classical statistical methods like autoregressive integrated moving average (ARIMA) \cite{cite_34} and Deep Learning (DL)-based methods such as Long Short-Term Memory (LSTM) \cite{cite_7} and Diffusion Convolutional Recurrent Neural Networks (DCRNN) \cite{cite_8}. However, both approaches only use temporal dependencies, overlooking spatial ones.

Graph Neural Networks (GNNs) \cite{cite_29} address these issues by modeling traffic data as a graph, where nodes represents a physical location, and edges spatial connections between these locations. Specifically, Spatio-Temporal Graph Neural Networks (ST-GNNs) \cite{cite_16} extend GNNs to capture both spatial and temporal dependencies, making them more effective than other DL-based approaches for traffic forecasting. Thus, numerous ST-GNN architectures have been developed and tested for this task \cite{cite_16}.

However, most previous works have focus on ST-GNN trained in centralized environments, where data from all sensors is continuously collected. But the task of collecting data, performing DL training and inference, and sending back commands is challenging to perform reliably in real-time in a centralized system. As sensors networks expand, scaling a central control system to handle the increased volume of data in real-time with low-latency becomes increasingly difficult. Furthermore, any issues in the central control system can easily result in a complete interruption of the service, requiring significant investments to maximize reliability. Given the key role played by mobility infrastructure in our societies, a centralized system can also become a significant target for hostile actors and a major cyber-weakness in strategic infrastructure management.

In this paper, we explore and adapt distributed training techniques for ST-GNNs in the smart mobility domain through semi-decentralized methods at the network edge, ensuring scalability and reliability. This approach utilizes geographically distributed cloudlets, hosted on edge devices with moderate computation and communication capabilities, as shown in Figure~\ref{fig:0.5}-a. Each cloudlet manages a subgraph of the overall traffic graph (Fig. \ref{fig:0.5}-b), shares node features necessary for local training step and model updates with other cloudlets to maintain consistency (Fig. \ref{fig:0.5}-c), and constructs ST-GNN subgraph required for training on its local nodes (Fig. \ref{fig:0.5}-d). The contributions of this paper can be summarized as follows:

\begin{itemize}
\item To our knowledge, we are the first to investigate semi-decentralize ST-GNN training with geographically distributed cloudlets
\item We develop a simulation framework for semi-decentralized ST-GNN training across cloudlets, allowing us to test different approaches.
\item Using our framework, we implement and compare four different training approaches---centralized, traditional FL, server-free FL, and Gossip Learning---providing the first comprehensive analysis of the benefits and drawback of these approaches for our targeted use-case, assessing their suitability for real-world deployment and informing future research endeavours.
\item We evaluate these approaches on two real-world datasets, METR-LA and PeMS-BAY \cite{cite_31}, across short-, mid-, and long-term traffic predictions, with a detailed analysis of model performance, cloudlet-specific metrics, communication overhead and computational costs.
\end{itemize}

Our experiments show that semi-decentralized approaches showed competitive performance against the centralized approach, especially for short-term prediction. Crucially, our analysis highlights the variation in model performance across different geographical areas due to region-specific traffic patterns, and the significant communication overhead and computational costs that arise from the large receptive field of GNNs, leading to substantial data transfers and increased computation of partial embeddings. This insight sheds light on a notable challenges in distributed ST-GNN training, which to our knowledge has not been explored in existing literature.

==> section_v3/2_preliminaries.tex <==
\section{Preliminaries}\label{sec:preliminares}
\subsection{Traffic prediction}
Traffic prediction is one of the most common and critical time-series forecasting tasks, as it estimates traffic metrics, such as speed, volume, and density to monitor current traffic conditions and predict future trends. It is generally classified into three forecasting horizons: short-term (15 min), mid-term (30 min), and long-term (60 min). In the context of ST-GNNs, the traffic system is represented as a spatial graph at the \textit{t}-th time step, denoted by $\mathcal{G}_t$ = ($\mathcal{V}_t$, $\mathcal{E}$, W), where $v_i, v_j\in \mathcal{V}_t$ is a finite set of nodes corresponding to observations from \textit{n} IoT-devices in the traffic network, $(v_i, v_j)\in \mathcal{E}$ is a set of edges connecting the IoT-devices, and $W\in \mathbb{R}^{n \times n}$ is a weighted adjacency matrix that encodes the spatial relationships between these IoT-devices. The spatial component is defined by the physical locations of IoT devices, while the temporal component arises from traffic features that evolve over time, influencing the graph's dynamics. While this work focuses on traffic prediction, methods for other smart mobility tasks can be generalized to this domain due to their shared reliance on spatio-temporal data. 

\subsection{Spatio-Temporal Graph Neural Networks}
ST-GNNs are DL models designed to capture both spatial and temporal dependencies in structured data, allowing it to simultaneously account for spatial correlations between nodes and temporal correlations over time, making it particularly suited for traffic prediction. By leveraging spatial dependencies, ST-GNNs provide a more accurate representation of how local traffic conditions at one location impact neighbouring locations.

Multiple ST-GNNs have been developed \cite{cite_16}, such as Graph Recurrent Network (GRN) \cite{cite_12}, Spatio-Temporal Graph Convolutional Network (ST-GCN) \cite{cite_13}, Graph Attention LSTM Network \cite{cite_14}, and many more \cite{cite_16}. Each technique addresses specific challenges or offers unique advantages over others. In this paper, we utilize ST-GCN due to their superior ability to handle traffic prediction tasks in the IoT context compared to other techniques. Experiments demonstrated that ST-GCN consistently outperforms other models in key evaluation metrics (MAE, MAPE, and RMSE) \cite{cite_13}.

\subsection{Traditional Federated Learning}
Traditional FL \cite{cite_30} is a collaborative machine learning (ML) approach where multiple clients work together to train a model, coordinated by a central aggregator. Instead of sharing raw data, which remains stored locally on each client device, the clients exchange only model updates with the server. These updates contain just the minimum information needed for the learning task, carefully scoped to limit the exposure of client data. The central aggregator then aggregates these focused updates as soon as they are received, ensuring that the learning process is both efficient and compliant with data minimization principles.

\subsection{Server-free Federated Learning}
Server-free FL \cite{cite_26} is a decentralized variant of the traditional FL approach. Unlike traditional FL, where a central aggregator is responsible for coordinating the model updates, server-free FL operates without a central entity. Instead, participating devices communicate directly with one another to exchange model parameters and perform local updates. After initializing their models, devices exchange model parameters with their neighbours, aggregate these received models with their own local model, and proceed to train on a subset of data. This iterative process allows for continuous refinement of models across the network, as the updated models are exchanged again between neighbouring devices.


\subsection{Gossip Learning}
Gossip Learning \cite{cite_27} is a decentralized protocol for training ML models in distributed settings without the need for a central coordinator. It is designed to be highly scalable and robust, allowing model updates to be propagated efficiently across a network of devices or nodes. Each device stores two models in its memory (as a FIFO buffer), typically representing the most recent models received from neighbouring devices. At each iteration of the gossip protocol, a device averages the weights of these two models to create an aggregated model. The device then performs one local training step using its own data, refining the aggregated model based on its local observations. Once the model is updated, the device forwards it to a randomly chosen device in the entire network. This process is repeated across the network, ensuring that models continuously evolve and improve as they traverse different nodes, collecting knowledge from the data they encounter at each location.

==> section_v3/3_methodology.tex <==
\section{Methodology}
\subsection{Scenario}
The traffic prediction scenario involves IoT-devices (i.e., sensors) deployed along highways to monitor real-time traffic conditions such as vehicle speed, volume, and density at fixed time intervals. To streamline data processing, IoT-devices are assigned to local base stations (BS), referred to as cloudlets, based on their physical proximity and communication range. The communication between IoT-devices and its BS is facilitated using Low-Power Wide-Area Network (LPWAN) protocols, such as LoRa or NB-IoT, which enable efficient, long-range, and low-power data transmission. Base stations, in addition to serving as communication hubs, are equipped with moderate computational resources. This existing computational power can be leveraged for training ML models, such as ST-GNNs.

\subsection{Distributed Training Setups}
We adopt a semi-decentralized ST-GNN architecture inspired by Nazzal et al. \cite{cite_25}, as it's one of the most effective architectures for distributed training. Figure~\ref{fig:0.5} shows key components of such architecture. In Fig.~\ref{fig:0.5}-a, traffic network is represented as a graph, where nodes correspond to IoT-devices, and edges represent road connections based on physical proximity. In Fig.~\ref{fig:0.5}-b, the graph is partitioned into subgraphs based on geographical proximity, each managed by a local cloudlet. In Fig.~\ref{fig:0.5}-c, cloudlets form a communication network for exchanging necessary node features and model updates. After communicating with each other, each cloudlet constructs ST-GNN subgraph required for training on its local nodes, as shown in Fig.~\ref{fig:0.5}-d.

Using this architecture, we evaluate four different training setups---centralized, traditional FL, server-free FL, and Gossip Learning---for ST-GNNs in the context of traffic prediction, with the centralized setup serving as a baseline for comparing the semi-decentralized approaches.

\subsection{GNN Partitioning in Distributed Training}
Partitioning the graph into subgraphs for local training in distributed GNN scenarios presents unique challenges due to their reliance on spatial dependencies. Unlike traditional ML models that process localized data independently, GNNs require information from neighbouring nodes to compute effective representations. Specifically, in an $\ell$-layer GNN, the representation of a node depends not only on its own features but also on the features of its $\ell$-hop neighbours.

This spatial dependency introduces a need for inter-cloudlet communication, as the required node features often extend beyond the boundaries of a single cloudlet's subgraph. Since IoT-devices typically have limited communication capabilities and cannot directly exchange data with distant cloudlets, the necessary node features are shared between the cloudlets themselves.

Each cloudlet, based on the underlying sensor network connectivity, is aware of which neighbouring cloudlets require its node features for local computations. When features are collected from the IoT-sensors, the cloudlet proactively broadcasts these features to the neighbouring cloudlets that need them for training (Fig.~\ref{fig:0.5}-d). This proactive exchange of node features ensures that each cloudlet has sufficient information to perform local computations without compromising the accuracy of the GNN model.

==> section_v3/4_experimental_setup.tex <==
\section{Experimental Setup}
\subsection{Datasets}
To evaluate the performance of our setups, we utilize two real-world public traffic datasets, PeMS-BAY\footnote{\label{footnote_1}Download link: \url{https://github.com/liyaguang/DCRNN}} and METR-LA\footref{footnote_1} \cite{cite_31}, which are collected by Caltrans performance measurement system. Both datasets consist of traffic data aggregated in 5-minute intervals, with each sensor collecting 288 data points per day. The details of datasets are listed in Table~\ref{table:1}.

% TABLE I
\begin{table}[htbp]
    \centering
    \caption{Details of METR-LA and PeMS-BAY}
    \begin{tabular}{c c c c c}
        \hline
        Datasets & Nodes & Interval & TimeSteps & Attribute \\
        \hline
        METR-LA & 207 & 5 min & 34,272 & Traffic speed \\
        PeMS-BAY & 325 & 5 min & 52,116 & Traffic speed \\
        \hline
    \end{tabular}
    \label{table:1}
\end{table}

The spatial adjacency matrix is constructed from the actual road network based on distance using the formula from ChebNet \cite{cite_28}. Specifically, it encodes the spatial relationships between nodes by assigning weights to edges based on the inverse of the pairwise distances between connected nodes, effectively capturing the connectivity and proximity of locations in the traffic network. Additionally, the data were preprocessed for efficient model training and evaluation. For example, if we want to utilize the historical data spanning one hour to predict the data the next hour, we pack the sequence data in group of 12 and convert it into an instance. The dataset was then split into training, validation, and test sets in a 70:15:15 ratio. Additionally, to mitigate the impact of varying data magnitudes, we applied standardization to normalize the original data values, reducing the impact of the large difference in value.

\subsection{Evaluation Metrics}
In our experiments, we evaluate the performance of different setups using Weighted Mean Absolute Percentage Error (WMAPE), in addition to the widely adopted Mean Absolute Error (MAE) and Root Mean Square Error (RMSE). We omit the formulas for MAE and RMSE due to their wide adoption. The WMAPE formula is as follows:

\begin{equation}
    \text{WMAPE}(\bm{x}, \bm{\hat{x}}) = \frac{\sum_{i}{\mid x_i - \hat{x}_i \mid}}{\sum_{i}{\hat{x}_i}} * 100\%,
\end{equation}

\noindent where $\bm{x} = x_1,\ldots,x_n$ denotes the ground truth values of vehicle speed, and $\bm{\hat{x}} = \hat{x}_1,\ldots,\hat{x}_n$ represents their predicted values.

We compute these metrics across three forecasting horizons—--short-, mid-, and long-term---to capture fluctuations in performance over time. For centralized and FL setups, the metrics are derived from the main server's aggregated model, while for server-free FL and Gossip Learning, they are computed as a weighted average of the individual cloudlet predictions. This ensures a consistent and fair comparison across all approaches.

% Figure 2
\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{figures/locations_metr-la_pems-bay_experiment_1_subplot.png}
  \caption{Sensor assignment to cloudlets based on communication range}
  \label{fig:2}
\end{figure}

\subsection{Experimental Setup}
% TABLE II
\begin{table*}[ht!]
\centering
\caption{Performance Comparison (MAE [$mile/h$]/RMSE [$mile^2/h^2$]/WMAPE [\%]) of four different setups}
\label{table:2}
\renewcommand{\arraystretch}{1.5} % Adjust row spacing for better readability
\begin{tabular}{l l ccc | ccc | ccc}
\hline\hline
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Setups} & \multicolumn{3}{c|}{15 min} & \multicolumn{3}{c|}{30 min} & \multicolumn{3}{c}{60 min} \\ 
\cline{3-11}
\multicolumn{2}{l}{} & MAE & RMSE & WMAPE & MAE & RMSE & WMAPE & MAE & RMSE & WMAPE \\ 
\hline\hline
\multirow{4}{*}{METR-LA} & Centralized             & 3.78 & 9.05      & 7.45 & 5.14 & 11.61       & 10.12 & 7.35 & 14.59      & 14.47 \\ \cline{3-11}
                                      & Traditional FL      & 3.97 & 9.01       & 7.82 & 5.40 & 11.41       & 10.63 & 7.82 & 14.48      & 15.40 \\ \cline{3-11}
                                      & Server-free FL          & 3.90 & 8.98 & 7.78     & 5.35 & 11.37 & 10.67     & 7.79 & 14.41 & 15.55 \\ \cline{3-11}
                                      & Gossip Learning         & 3.88 & 9.04 & 7.74     & 5.43 & 11.35 & 10.85     & 7.56 & 14.42 & 15.10 \\ 
\hline\hline
\multirow{4}{*}{PeMS-BAY} & Centralized             & 1.48 & 3.09      & 2.38 & 1.97 & 4.23      & 3.17 & 2.59 & 5.41      & 4.17 \\ \cline{3-11}
                                       & Traditional FL      & 1.50 & 3.12      & 2.42 & 2.03 & 4.29      & 3.27 & 2.67 & 5.51      & 4.29 \\ \cline{3-11}
                                       & Server-free FL          & 1.50 & 3.12 & 2.42    & 2.01 & 4.25 & 3.23      & 2.65 & 5.44 & 4.28 \\ \cline{3-11}
                                       & Gossip Learning         & 1.51 & 3.12 & 2.43    & 2.03 & 4.28 & 3.26      & 2.63 & 5.39 & 4.24 \\ 
\hline\hline
\end{tabular}
\end{table*}
